Shaping mmWave Wireless Channel via Multi-Beam Design using Reconfigurable Intelligent Surfaces

Millimeter-wave (mmWave) communications is considered as a key enabler towards the realization of next-generation wireless networks, due to the abundance of available spectrum at mmWave frequencies. However, mmWave suffers from high free-space path-loss and poor scattering resulting in mostly line-of-sight (LoS) channels which result in a lack of coverage. Reconfigurable intelligent surfaces (RIS), as a new paradigm, have the potential to fill the coverage holes by shaping the wireless channel. In this paper, we propose a novel approach for designing RIS with elements arranged in a uniform planar array (UPA) structure. In what we refer to as multi-beamforming, We propose and design RIS such that the reflected beam comprises multiple disjoint lobes. Moreover, the beams have optimized gain within the desired angular coverage with fairly sharp edges avoiding power leakage to other regions. We provide a closed-form low-complexity solution for the multi-beamforming design. We confirm our theoretical results by numerical analysis.

==> UPA_Codebook.tex <==
\subsection{UPA Codebook Design Prolem}

Suppose an $M_h \times M_v$ UPA is placed at the $x-z$ plane, and let $M = M_h M_v$. Let the distance between the antennas that are placed parallel to $z$ axis, be $d_z$, and $d_x$ respectively. One can define,

\begin{align}
\mathbf{d}_{M_{a}}\left(\psi_{a}\right) = \left[1, e^{j \psi_{a}} \cdots e^{j\left(M_{a}-1\right) \psi_{a}}\right]^{T} \in \mathbb{C}^{M_{a}}
\end{align}
where, $\psi_{h}=\frac{2 \pi d_{x}}{\lambda} \sin \theta \cos \phi \text { and } \psi_{v}=\frac{2 \pi d_{z}}{\lambda} \sin \phi$, and $a$ takes value in the set $\{v, h\}$.  
The array response vector is then defined as 

\begin{align}
    \mathbf{d}_{M}\left(\psi_{v}, \psi_{h}\right) =
    \mathbf{d}_{M_{v}}\left(\psi_{v}\right) \otimes
    \mathbf{d}_{M_{h}}\left(\psi_{h}\right)  \in \mathbb{C}^{M}
\end{align}
Let $\mathcal{B}_s$ be the angular range under cover in the $(\psi_h, \psi_v)$ domain. We have, 

\begin{equation}
    \mathcal{B}^\psi_{s} \doteq\left[-\psi_h^{\mathrm{B}}, \psi_h^{\mathrm{B}}\right) \times\left[-\psi_v^{\mathrm{B}}, \psi_v^{\mathrm{B}}\right)
\end{equation}

% \begin{equation}
%     \mathcal{B}_{s} \doteq \left[-\phi^{\mathrm{B}}, \phi^{\mathrm{B}}\right)
%     \times \left[-\theta^{\mathrm{B}}, \theta^{\mathrm{B}}\right) \label{range_angle}
% \end{equation}

% Notation $\psi^{p,q}_{h}[1:L_h,1 :L_v], \psi^{p,q}_{v}[1:L_v]$

Let us uniformly divide the angular range  into $Q=Q_{v} Q_{h}$ subregions. For each subregion we have, 

% $$ \mathcal{B}_{p, q} =  \omega_{\phi, p} \times \omega_{\theta, q}$$

% Let $\Delta_{\theta} =  2 \theta^{\mathrm{B}} / Q_{v}$, and $\Delta_\phi =  2 \phi^{\mathrm{B}} / Q_{h}$ be the length of each sub-interval along axis $\theta$, and $\phi$. We have $\omega_{\theta, q} = [\theta_{q-1}, \theta_q)$, and, $\omega_{\phi, p} = [\phi_{p-1},\phi_p)$ where  $\theta_q = -\theta^B + q\Delta_\theta$, and $\phi_p = -\phi^B + p\Delta_\phi$. 


$$ \mathcal{B}_{ p, q} \doteq \nu_{v}^{p, q} \times \nu_{h}^ {p, q}$$

% We can then write for each $v_{a, b}$, i.e the $b$-th sub-interval along axis $a$,

% \begin{equation}
%     \nu_{v, p} =-\psi_{a}^{\mathrm{B}}+(b-1)\Delta_{a}+\left[0, \Delta_{a}\right)
% \end{equation}

Define the reference gain at $(\psi_{h}, \psi_{v}) $ as, 

\begin{equation}
    G\left(\psi_{v}, \psi_{h}, \mathbf{c}\right) =\left|\left(\mathbf{d}_{M_{v}}\left(\psi_{v}\right)\otimes\mathbf{d}_{M_{h}}\left(\psi_{h}\right)  \right)^{H} \mathbf{c}\right|^{2}
\end{equation}

It is straightforward to show that, 

\begin{equation}
    \int_{-\pi}^{\pi} \int_{-\pi}^{\pi} G\left(\psi_{v}, \psi_{h}, \mathbf{c}\right) d \psi_{v} d \psi_{h}={(2 \pi)^{2}}
\end{equation}

Therefore, for every interval $\mathcal{B}_{ p, q}$ we can derive the ideal gain expression as, 

\begin{equation}
    G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)=G_{p,q} \mathds{1}_{\mathcal{B}^\psi_{p, q}}\left(\psi_{v}, \psi_{h}\right)
\end{equation}

where $G_{q,p} = \frac{(2\pi)^2}{\delta_{p,q}}$, where $\delta_{p,q}$ is the area of the interval $\mathcal{B}^\psi_{p,q}$. We can write $\delta_{p,q} = \delta_v\delta_h = (\frac{2\psi^B_v}{Q_v})(\frac{2\psi^B_h}{Q_h})$. Therefore, We define the codebook design problem under the UPA structure as follows. 
% where $G_{q,p} = \frac{(2\pi)^2}{\delta^{p,q}_h\delta^p_v}$, $\delta^p_v = \psi^p_v - \psi^{p-1}_v $, and $\delta^{q, p}_h = \psi^{q,p}_h - \psi^{q-1, p}_h $. Also, let us define $\delta_{q,p} = \delta^{q, p}_h\delta^p_v$. 



\begin{align}
& \c^{opt}_{p, q} = \nonumber\\&\underset{\c, \|\c\|=1}{\arg \min } \iint_{\mathcal{B}_{s}}\left|G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)-G\left(\psi_{v}, \psi_{h}, \c\right)\right| d \psi_{v} d \psi_{h} \label{init_opt}
\end{align}

By partitioning the range of $(\psi_h, \psi_v)$ into the pre-defined intervals, we can rewrite the optimization problem as follows, 

\begin{align}
& \c^{opt}_{p, q} = \underset{\c, \|\c\|=1}{\arg \min }\nonumber\\& \sum_{r=1}^{Q_v}\sum_{s=1}^{Q_h}\iint_{\mathcal{B}^{\psi}_{r,s}}\left|G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)-G\left(\psi_{v}, \psi_{h}, \c\right)\right| d \psi_{v} d \psi_{h} \nonumber\\&
 = \underset{L_h, L_v \rightarrow \infty}{\lim}\sum_{r=1}^{Q_v}\sum_{s=1}^{Q_h}\sum_{l_v =1}^{L_v}\sum_{l_h =1}^{L_h}\frac{\delta_v\delta_h}{L_hL_v}\nonumber\\&
\left|G_{p, q}^{\text {ideal }}\left(\psi^{r,s}_{v}[l_v], \psi^{r,s}_{h}[l_h]\right)-G\left(\psi^{r,s}_{v}[l_v], \psi^{r,s}_{h}[l_h], \c\right)\right| \label{alternative_opt}
\end{align}
where, 

\begin{align}
    &\psi^{r,s}_v[l_v] = \psi^{r-1, s}_v + l_v\frac{\delta_v}{L_v}\nonumber\\
    &\psi^{r,s}_h[l_h] = \psi^{r, s-1}_h + l_h\frac{\delta_h}{L_h}
\end{align}

We can rewrite the optimization problem \eqref{alternative_opt} as, 

\begin{align}
    \c_{p,q}^{opt}=\arg \min _{\c, \|\c\|=1} \underset{L_h, L_v \rightarrow \infty}{\lim}\frac{1}{L_hL_v}\left\|\mathbf{G}^{\text {ideal }}_{p,q}-\mathbf{G}(\c)\right\|
\end{align}


where, 

\begin{align}
    \mathbf{G}(\c) =& \delta_v\delta_h\left[G\left(\psi_{v}^{1,1}[1], \psi_{h}^{1,1}[1], \c\right) \cdots \right. \nonumber\\ &\left. G\left(\psi_{v}^{Q_{v}, Q_{h}}\left[L_{v}\right], \psi_{h}^{Q_{v}, Q_{h}}\left[L_{h}\right], \c\right)\right]^{T} 
\end{align}

and, 

\begin{align}
    \mathbf{G}^{\text {ideal }}_{ p, q} =& \delta_v\delta_h\left[G^{\text {ideal }}_{ p, q}\left(\psi_{v}^{1,1}[1], \psi_{h}^{1,1}[1] \right) \cdots \right. \nonumber\\ &\left. G^{\text {ideal }}_{ p, q}\left(\psi_{v}^{Q_{v}, Q_{h}}\left[L_{v}\right], \psi_{h}^{Q_{v}, Q_{h}}\left[L_{h}\right]\right)\right]^{T} 
\end{align}


% \begin{align}
%      &\mathbf{G}^{\text {ideal }}_{ q, p}= \nonumber\\&\left[{\delta_{1,1}} G^{\text {ideal }} _{q, p}\left(\psi^{1}_{h}[1], \psi^{1}_{v}[1], \c\right) \ldots {\delta_{Q_h, Q_v}}G^{\text {ideal }} _{q, p}\left(\psi^{Q_h}_{h}[L_h], \psi^{Q_v}_{v}[L_v], \c\right)\right]^{T} 
% \end{align}


Note that we can write, 

\begin{align}
    \mathbf{G}^{\text{ideal }}_{p,q} = \delta_v\delta_h\frac{{(2\pi)}^2}{\delta_v\delta_h} \left(\e_{p,q} \otimes \mathbf{1}_{L, 1}\right)
\end{align}


with $\mathbf{e}_{p,q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $(p,q)$-th axis among $Q$ ones. 








Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any equal gain $\mathbf{g} \in \mathbb{C}^L$. Therefore, we can write: 

% $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$


\begin{align}
\mathbf{G}^{\text {ideal }}_{p,q} &={{(2\pi)}^2}\left(\mathbf{e}_{p,q} \otimes(\mathbf{g} \odot \mathbf{g}^{*})\right) \nonumber\\
&=\left({{2\pi}}\left(\mathbf{e}_{p,q} \otimes \mathbf{g}\right)\right) \odot \left({{2\pi}}\left(\mathbf{e}_{p,q} \otimes \mathbf{g}\right)\right)^* \label{g_id_q_equivalent}
\end{align}

Also, note that we can write, 

% \begin{align}
%     \mathbf{G}(\c)=\left(\left(\mathbf{D}_{h}^{H} \otimes \mathbf{D}_{v}^{H}\right) \c\right) \odot\left(\left(\mathbf{D}_{h}^{H} \otimes \mathbf{D}_{v}^{H}\right) \c\right)^{*}
% \end{align}
\begin{align}
    \mathbf{G}(\c)=\left(\D^H \c\right) \odot\left(\D^H \c\right)^{*}
\end{align}

\noindent where, $\D^H = \sqrt{\delta_v\delta_h}(\mathbf{D}_{v}^{H} \otimes \mathbf{D}_{h}^{H})$, and for $a \in \{v,h\}$, we have, 

\begin{align}
\mathbf{D}_{a} &=\left[\mathbf{D}_{a, 1}, \cdots, \mathbf{D}_{a, Q_{a}}\right] \in \mathbb{C}^{M_{a} \times L_{a} Q_{a}} \\
\mathbf{D}_{a, b} &=\left[\mathbf{d}_{M_{a}}\left(\psi_{a}^{b}[1]\right), \cdots, \mathbf{d}_{M_{a}}\left(\psi_{a}^{b}\left[L_{a}\right]\right)\right] \in \mathbb{C}^{M_{a} \times L_{a}}
\end{align}




% where 

% \begin{align}
%     \D = \left[D^{1,1}_{vh}, \cdots, D^{Q_v,Q_h}_{vh}\right] \in \mathbb{C}^{M_vM_h\times L_vL_hQ_vQ_h}
% \end{align}

% \begin{align}
% % &\mathbf{D}_{v} =\left[\mathbf{D}_{v, 1}, \cdots, \mathbf{D}_{v, Q_{v}}\right] \in \mathbb{C}^{M_{v} \times L_{v} Q_{v}} \\
% % &\mathbf{D}_{h} =\left[\mathbf{D}_{h, 1}, \cdots, \mathbf{D}_{h, Q_{h}}\right] \in \mathbb{C}^{M_{h} \times L_{h} Q_{h}} \\
% % &\mathbf{D}_{v, p} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right)\right] \in \mathbb{C}^{M_{v} \times L_{v}}\\
% % &\mathbf{D}_{h, q} =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1]\right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right]\right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% &\mathbf{D}_{h, q}(\chi) =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1], \chi \right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right], \chi \right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% &\mathbf{D}_{vh, p,q} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right) \otimes \mathbf{D}_{h, q}(\psi_{v}^{p}[1]), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right) \otimes \mathbf{D}_{h, q}(\psi_{v}^{p}\left[L_{v}\right]) \right] \in \mathbb{C}^{M_{v}M_{h} \times L_{v}L_{h}}
% \end{align}

% \begin{align}
% % &\mathbf{D}_{v} =\left[\mathbf{D}_{v, 1}, \cdots, \mathbf{D}_{v, Q_{v}}\right] \in \mathbb{C}^{M_{v} \times L_{v} Q_{v}} \\
% % &\mathbf{D}_{h} =\left[\mathbf{D}_{h, 1}, \cdots, \mathbf{D}_{h, Q_{h}}\right] \in \mathbb{C}^{M_{h} \times L_{h} Q_{h}} \\
% % &\mathbf{D}_{v, p} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right)\right] \in \mathbb{C}^{M_{v} \times L_{v}}\\
% % &\mathbf{D}_{h, q} =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1]\right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right]\right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% \mathbf{D}^{p,q}_{h}(\ell) =&\sqrt{\delta_v^{p}\delta^{p,q,\ell}_h}\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{p,q}[\ell][1] \right), \cdots, \right.\nonumber\\&\left. \mathbf{d}_{M_{h}}\left(\psi_{h}^{p,q}\left[\ell] [L_{h} \right] \right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}, 
% \end{align}

% \begin{align}
%     \mathbf{D}_{vh}^{p,q} =&\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p,q}[1]\right) \otimes \mathbf{D}_{h}^{p,q}(1), \cdots, \right.\nonumber\\&\left. \mathbf{d}_{M_{v}}\left(\psi_{v}^{p,q}\left[L_{v}\right]\right) \otimes \mathbf{D}_{h}^{p,q}(L_{v}) \right] \in \mathbb{C}^{M_{v}M_{h} \times L_{v}L_{h}}
% \end{align}

\begin{problem}
Given an equal-gain vector $\g_{p,q} \in \mathbb{C}^L$, $(p,q) \in \{(1,1), \cdots, (Q_v, Q_h)\}$, find vector $\c_{p,q} \in \mathbb{C}^{M_t}$ such that
\begin{align}
&\c_{p,q}=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\rightarrow \infty} \left\|{{2\pi}}\left(\mathbf{e}_{p,q} \otimes \mathbf{g}\right)- \D^H \c\right\|^{2} \label{obj_func}
\end{align}
\label{main_problem_UPA}
\end{problem}


Note that the solution to problem \ref{main_problem_UPA} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity. For each $L$ we find that,
 \begin{align}
 {\c}^{(L)}_{p,q} &= {{{2\pi}}}(\D \D^H)^{-1} \D  \left(\mathbf{e}_{p,q} \otimes \mathbf{g}_{p,q}\right) \nonumber\\& =\sigma \D_{p,q}\mathbf{g}_{p,q}
\end{align}
where $\sigma = \frac{2\pi \sqrt{\delta_{v}\delta_{h}}}{LQ\delta_{v}\delta_{h}} = \frac{2\pi}{LQ\sqrt{\delta_v\delta_h}}$, noting that it holds that, 

Noting that it holds that, 

\begin{align}
    (\D\D^H) = \left(L\sum_{(p,q)= (1,1)}^{(Q_h, Q_v)}\sum_{(l_v,l_h)= (1,1)}^{(L_h, L_v)} \delta_{v}\delta_{h}\right)\I_{M_t}
\end{align}

\begin{problem}
Find equal-gain $\g_{p,q} \in \mathbb{C}^L$, $(p,q) = (1,1), \ldots, (Q_h, Q_v)$, such that
\begin{equation}
 \g_{q,p} = \underset{\g}{\arg\min }\left\| abs(\D^H \c_{p,q})- {2\pi} abs(\mathbf{e}_{p,q} \otimes \mathbf{g})\right\|^{2} \label{g_final_eq}
\end{equation} 
where $abs(.)$ denotes the element-wise absolute value of a vector.
\label{g_problem}
\end{problem}


\begin{proposition}
The minimizer of \eqref{g_simple_final_eq} is in the form $\g_q = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha_v^{\eta (L_v -1)}\alpha_h^{\eta (L_h -1)} \end{array}}\right]^T$ for some $\eta$ where $\alpha_v = e^{j(\frac{\eta_v}{L_v})}$ and $\alpha_h = e^{j(\frac{\eta_h}{L_h})}$. \label{proposiiton_g}
\end{proposition}

 \begin{align}
     {\c_{p,q}}^{(L)} & = \sigma \sum_{(l_v, l_h)=(1,1)}^{(L_v, L_h)}g_{p,q, l}\mathbf{d}_{M_t}\left(\psi^{p}_{v}[l_v], \psi^{q}_{h}[l_h]\right)  \nonumber\\
     & = \sigma \sum_{l=1}^L g_{q,p,l}\left[{\begin{array}{ccc}
     1 &\cdots & e^{j\phi_{p,q}^{M_v-1, M_h-1}}\\
     \end{array}}\right]^T   
    %  \nonumber\\& = \left[{\begin{array}{ccc}
    %  \sigma\sum_{l=1}^L g_{q, p, l}& \cdots & \sigma\sum_{l=1}^L g_{q,p, l}e^{j\left((M_h-1)\psi^q_{h}[l] + (M_v-1)\psi^p_{v}[l]\right)}\\
    %  \end{array}}\right]^T
\end{align}

where $ \phi_{p,q}^{m_v, m_h} = \left( m_v\psi^{p}_{v}[l_v] + m_h\psi^{q}_{h}[l_h]\right)$. We can then write 

\begin{align}
    c_{p,q, m_v, m_h} &= \nonumber\\& \lim_{L_h, L_v\rightarrow \infty} \frac{1}{L_hL_v}\sum_{(l_h, l_v)=(1,1)}^{(L_h, L_v)} g_{p,q, l_v, l_h}e^{j\phi_{p,q}^{M_v-1, M_h-1}}
\end{align}


\begin{align}
    c_{p,q, m_v, m_h} &=  \lim_{L_h, L_v\rightarrow \infty} \frac{1}{L_hL_v}\sum_{(l_h, l_v)=(1,1)}^{(L_h, L_v)} g_{p,q, l_v, l_h}\nonumber \\&e^{j\left(m_v(\psi^{p-1}_{v}+l_v\frac{\delta_v}{L_v})+ m_h(\psi^{q-1}_{h} + l_h\frac{\delta_h}{L_h}) \right)}
\end{align}


\begin{align}
    c_{p,q, m_v, m_h} =&  \frac{2\pi}{Q}e^{j\phi_{p-1, q-1}^{m_v, m_h}}
    \left(\frac{1}{L_v}\lim_{ L_v\rightarrow \infty} \sum_{l_v=1}^{L_v} e^{j\frac{\eta_v+ m_v\delta_v}{L_v} l_v}\right) \nonumber\\&
    \left(\frac{1}{L_h}\lim_{ L_h\rightarrow \infty} \sum_{l_h=1}^{L_h} e^{j\frac{\eta_h+ m_h\delta_h}{L_h} l_h}\right)
\end{align}

\begin{align}
    c_{p,q, m_v, m_h} &=  \frac{2\pi}{Q}e^{j\phi_{p-1, q-1}^{m_v, m_h}}
    \int_{0}^{1} e^{j\xi_v x}dx\int_{0}^{1} e^{j\xi_h x}dx \nonumber\\&
    = \frac{2\pi}{Q}e^{j(\phi_{p-1, q-1}^{m_v, m_h}+ \frac{\xi_v+\xi_h}{2})} sinc(\frac{\xi_v}{2\pi})sinc(\frac{\xi_h}{2\pi})
\end{align}

with $\xi_a = {\delta_a}{m_a} + \eta_a$, where $a\in \{v,h\}$. 
% Therefore, it. holds that, 

% \begin{align}
%     c_{p,q, m_v, m_h} &=  \lim_{ L_v\rightarrow \infty} \frac{\delta^p_v}{L_v}\sum_{l_v=1}^{L_v} e^{j(m_v(\psi^{p-1,q}_{v}+l_v\frac{\delta^p_v}{L_v}) + x\eta\frac{l_v}{L_v})} \delta^{p,q,l_v}_h e^{jm_h\psi^{p,q-1}_{h}[l_v]}sinc(\frac{\xi}{2\pi}) 
% \end{align}

==> composite.tex <==
\subsection{Composite Codebook Design Problem}

Let us define a \textit{composite beam} $\omega_k$ as a union of multiple disjoint, possibly non-neighboring beams $\nu_{q} \text { for } q \in \mathcal{Q} = \left\{1, \cdots, Q\right\}$. Let $\mathcal{C'}=\left\{\mathbf{c}_{1}, \cdots, \mathbf{c}_{K}\right\}$ be the codebook corresponding to the composite problem.

% $$\bigcup_{k = 1}^{2^{B'}}{\omega_k} = [-\pi, \pi], \quad \text{and} \quad \omega_k \cap \omega_l = \emptyset, \quad \forall k\neq l.$$

Moreover, define for each composite beam $\omega_k$ the set $\mathcal{W}_k \subseteq \mathcal{Q}$ to be the set of indices of the single beams that form $\omega_k$. i.e. $\mathcal{W}_k = \{q \in \mathcal{Q}: v_q \subseteq \omega_k\}$. 
For any codeword $\c$, it holds that, 

\begin{equation}
    \int_{-\pi}^{\pi} G(\psi, \mathbf{c}) d \psi=2 \pi\|\mathbf{c}\|^{2}=2 \pi
\end{equation}
We have then for the ideal gain corresponding to  each codeword $\textbf{c}_k$, 

\begin{align}
&\int_{-\pi}^{\pi} G_{\text {ideal }, k}(\psi) d \psi =\int_{\omega_{k}} t d \psi+\int_{[-\pi, \pi] \backslash \omega_{k}} 0 d \psi \nonumber\\
&= \sum_{q \in {\mathcal{W}_k}}{\int_{\nu_{q}} t d \psi} = \sum_{q \in \mathcal{W}_k}\delta_q t=2 \pi \label{composite}
\end{align}

Therefore, $t = \frac{2 \pi}{\Delta_k}$, where $\Delta_k = \sum_{q \in \mathcal{W}_k}\delta_q$. It follows that, 

\begin{equation}
    G_{\text {ideal }, k}(\psi)=\frac{2 \pi}{\Delta_k} \mathds{1}_{\omega_{k}}(\psi), \quad \psi \in[-\pi, \pi] \label{composite_ideal_gain}
\end{equation}

The new MSE problem for the $k$-th codeword can therefore be written as follows.



\begin{align}
\c_k^{opt} &=\underset{\c, \|\c\|=1}{\arg \min } \int_{-\pi}^{\pi}\left|G_{\text {ideal }, k}(\psi)-G(\psi, \c)\right| d \psi 
\end{align}




By uniformly sampling on the range of   we can rewrite
the optimization problem as follows,

\begin{align}
    \c_k^{opt} &= \nonumber \\&\underset{\c, \|\c\|=1}{\arg \min }\left[\lim _{L \rightarrow \infty} \sum_{p=1}^{Q} \delta_p\sum_{\ell=1}^{L} \frac{\left|G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \c\right)\right|}{L}\right]\label{composite_MSE}
\end{align}

 where, for $q = 1 \ldots Q$, 
 $$\delta_q = \psi_{q}-\psi_{q-1}, \quad \psi_{q, \ell}=\psi_{q-1}+\frac{\delta_q(\ell-0.5)}{L} $$

We can rewrite equation \eqref{composite_MSE} as follows, 

\begin{align}
 &\c_k^{opt} = \underset{\c,  \|\c\|=1}{\arg \min } \lim_{L\rightarrow \infty}\frac{1}{L}\left\|\mathbf{G}_{\text {ideal }, k}-\mathbf{G}(\c)\right\| \label{init_opt}
 \end{align}
 
 where,  $$\mathbf{G}(\c)=\left[{\delta_1} G\left(\psi_{1,1}, \c\right) \ldots {\delta_{Q}}G\left(\psi_{Q, L}, \c\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

and, 
$$ \mathbf{G}_{\text {ideal }, k}=\left[{\delta_1} G_{\text {ideal }, k}\left(\psi_{1,1}\right) \ldots {\delta_{Q}}G_{\text {ideal }, k}\left(\psi_{Q, L}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$


Note that it holds that 

\begin{equation}
    \mathbf{G}_{\text {ideal },k}=\sum_{q \in \mathcal{W}_k}\delta_q\frac{2\pi}{\Delta_k}\left(\mathbf{e}_{q} \otimes \mathbf{1}_{L, 1}\right) \label{ideal}
\end{equation}

with $\mathbf{e}_{q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $q$-th axis among $Q$ ones. Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any equal gain $\mathbf{g} \in \mathbb{C}^L$. Therefore, for a suitable choice of $\g$ we can write: 

% $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$


\begin{align}
\mathbf{G}_{\text {ideal }, k} &= \sum_{q \in \mathcal{W}_k}\gamma_q\left(\mathbf{e}_{q} \otimes\left(\mathbf{g} \odot \mathbf{g}^{*}\right)\right) \nonumber\\
&=\sum_{q \in \mathcal{W}_k}\left(\sqrt{\gamma_q}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right)\right) \odot\left(\sqrt{{\gamma_q}}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right)\right)^{*} \nonumber\\
&=\left(\sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)  \odot \left(\sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)^{*} \label{final_gik}
\end{align}




















% \begin{align}
% \left(\mathbf{F}_{k}, \mathbf{v}_{k}\right) &=\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \sum_{p=1}^{Q} \sum_{\ell=1}^{L}\left|G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \mathbf{F} \mathbf{v}\right)\right|^{2} \nonumber\\
% &=\underset{\mathbf{F}, \mathbf{v}}{\arg \min }\lim_{L\longrightarrow \infty} \frac{1}{L}\left\|\mathbf{G}_{\text {ideal }, k}-\mathbf{G}(\mathbf{F} \mathbf{v})\right\|_{2}^{2} \label{init_opt}
% \end{align}

% where,  $$\mathbf{G}(\mathbf{F} \mathbf{v})=\left[G\left(\psi_{1,1}, \mathbf{F} \mathbf{v}\right) \cdots G\left(\psi_{Q, L}, \mathbf{F} \mathbf{v}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% and, 
% $$ \mathbf{G}_{\text {ideal }, k}=\left[G_{\text {ideal }, k}\left(\psi_{1,1}\right) \cdots G_{\text {ideal }, k}\left(\psi_{Q, L}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% Note that we can write using the definition of $\mathcal{W}_k$ that, 

% $$G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)=\left\{\begin{array}{ll}
% \frac{Q}{|\mathcal{W}_k| M_{t}}, & p \in \mathcal{W}_k \\
% 0, & p \notin \mathcal{W}_k 
% \end{array},\right.$$

% Or in the matrix form, 

% \begin{align}
%     &\mathbf{G}_{\text {ideal }, k}=\frac{Q}{|\mathcal{W}_k| M_{t}}\left((\bigoplus_{q \in \mathcal{W}_k}{\mathbf{e}_{q}}) \otimes \mathbf{1}_{L, 1}\right)  \nonumber \\ 
%     & = \sum_{q \in \mathcal{W}_k}{\frac{Q}{|\mathcal{W}_k| M_{t}}\left(\mathbf{e}_{q} \otimes \mathbf{1}_{L, 1}\right)} \label{G_ideal_k}
% \end{align}

% with $\mathbf{e}_{q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $q$-th axis among $Q$ ones. Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any $\mathbf{g} \in \mathcal{G}_L$, where, 

% $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$



% Therefore, equation \eqref{G_ideal_k} can be rewritten as:
% \begin{align}
% &\mathbf{G}_{\text {ideal }, k} = \sum_{q \in \mathcal{W}_k}\frac{Q}{|\mathcal{W}_k| M_{t}}\left(\mathbf{e}_{q} \otimes\left(\mathbf{g}_q \odot \mathbf{g}_q^{*}\right)\right) \nonumber\\
% &=\sum_{q \in \mathcal{W}_k}\left(\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right) \odot\left(\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)^{*} \nonumber\\
% &=\left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)  \odot \left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)^{*} \label{final_gik}
% \end{align}

% where $\sigma = \sqrt{\frac{Q}{|\mathcal{W}_k|M_{t}}}$. 

Similarly, it is straightforward to observe,


\begin{align}
\mathbf{G}(\c) &=\left(\mathbf{D}^{H} \c\right) \odot\left(\mathbf{D}^{H} \c\right)^{*} \label{dc}
\end{align}
where $\mathbf{D} =\left[\sqrt{\delta_1}\mathbf{D}_{1} \cdots \sqrt{\delta_{Q}}\mathbf{D}_{Q} \right] \in \mathbb{C}^{M_{t} \times L Q}$, and 
$\mathbf{D}_{q}=\left[\mathbf{d}_{M_{t}}\left(\psi_{q, 1}\right) \cdots \mathbf{d}_{M_{t}}\left(\psi_{q, L}\right)\right] \in \mathbb{C}^{M_{t} \times L}.$
 







% On the other hand note that $\mathbf{G}(\mathbf{F} \mathbf{v})$ can be written as,


% \begin{equation}
%     \mathbf{G}(\mathbf{F} \mathbf{v}) =\left(\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right) \odot\left(\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right)^{*}\label{dfv_decomp}
% \end{equation}

% where, 
% $$\mathbf{D} =\left[\mathbf{D}_{1} \cdots \mathbf{D}_{Q}\right] \in \mathbb{C}^{M_{t} \times L Q}$$

% and, $\mathbf{D}_{q}=\left[\mathbf{d}_{M_{t}}\left(\psi_{q, 1}\right) \cdots \mathbf{d}_{M_{t}}\left(\psi_{q, L}\right)\right] \in \mathbb{C}^{M_{t} \times L}$. 

Comparing the expressions \eqref{init_opt}, \eqref{final_gik}, and \eqref{dc}, one can show that the optimal choice of $\c_q$ in \eqref{init_opt} is the solution to the following optimization problem for a proper choice of $\g_q$. 
\begin{problem}
Given an equal-gain vector $\g_q \in \mathbb{C}^L$, $q \in \{1, \cdots, Q\}$, find vector $\c_q \in \mathbb{C}^{M_t}$ such that
\begin{align}
&\c_q=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\rightarrow \infty} \left\|\sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)- \mathbf{D}^{H} \c\right\|^{2} \label{obj_func}
\end{align}
\label{main_problem}
\end{problem}


However, we now need to find the optimal choice of $\g_q$ that minimizes the objective in \eqref{init_opt}. Using \eqref{final_gik}, and \eqref{dc}, we have the following optimization problem.
\begin{problem}
Find a set of equal-gain $\g_q \in \mathbb{C}^L$, i.e. $\mathcal{G}_k$ such that
\begin{equation}
 \mathcal{G}_k = \underset{\mathcal{G}}{\arg\min }\left\| abs(\D^H \c_q)- abs(\sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}(\mathbf{e}_{q} \otimes \mathbf{g}_q))\right\|^{2} \label{g_final_eq}
\end{equation} 
where $\mathcal{G}_k = \{\g_q| q \in \mathcal{W}_k\}$, and $abs(.)$ denotes the element-wise absolute value of a vector.
\label{g_problem}
\end{problem}

Hence, the codebook design for a system with full-digital beamforming capability is found by solving Problem~\ref{main_problem} for proper choice of $\g_q$ obtained as a solution to Problem ~\ref{g_problem}. The codebook for Hybrid beamforming, is then found as
\begin{align}
    \underset{\mathbf{F}_{q},\mathbf{v}_{q}}{\arg\min } \|\mathbf{F}_{q}\mathbf{v}_{q} - \c_q\|^2
\end{align}
where the columns of $\F_q \in \mathbb{C}^{M_t \times N_{RF}}$ are equal-gain vectors and $\v_q \in \mathbb{C}^{N_{RF}}$. The solution may be obtained using simple, yet effective suboptimal algorithm such as orthogonal matching pursuit (OMP) \cite{love15}\cite{noh17}\cite{Hussain17}. In the next section we continue with the solution of Problem~\ref{main_problem}, and~\ref{g_problem}.





% Comparing the expressions in equations \eqref{final_gik}, and, \eqref{dc}, a perfect solution to the optimization problem in \eqref{init_opt}, could be a pair $\textbf{(F, v)}$, for which the following equality holds.  



% \begin{align}
%     \mathbf{D}^{H} \mathbf{F} \mathbf{v}=\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right) \label{potential_answer}
% \end{align}

% However, we have that $M_t > N_{RF}$ and therefore, the matrix $\textbf{D}^H \textbf{F}$ may not be full-rank, resulting in the RHS of equation \eqref{potential_answer} being in the null space of LHS. Therefore, given some $\g_q \in \mathcal{G}_L$ we formulate the following two-step optimization problem to search for $\textbf{(F, v)}$ that gets as close as possible to the desired value. 

% \begin{problem}

% a) For all $q \in \{1, \cdots, Q\}$, given $\g_q \in \mathcal{G}_L$, find the unit-norm vector $\c_q \in \mathbb{C}^{M_t}$ such that
% \begin{align}
% &\c^{|\g_q}_q=\underset{\c}{\arg \min } \lim_{L\longrightarrow \infty} \frac{1}{L}\left\|\left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)- \mathbf{D}^{H} \c\right\|_{2}^{2} \label{obj_func}
% \end{align}

% \noindent
% b) For every given $\c_q$, find $\F_q \in \mathbb{C}^{M_t \times N_{RF}}$ , and $\v_q \in \mathbb{C}^{N_RF}$ that satisfy $\mathbf{F}_{q}\mathbf{v}_{q} = \c_q$ the condition $\f_n \in \mathcal{B}_{M_t}$ as in equation \eqref{f_constant_gain}. 

% \begin{align}
%     \mathbf{F}_{\mid \g_q}\mathbf{v}_{\mid \g_q} = \c_q
% \end{align}

% \end{problem}



Note that the solution to problem \ref{main_problem} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity. For each $L$ we find that,
 \begin{align}
& {\c}^{(L)}_k = \sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}(\D \D^H)^{-1} \D  \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
& {\c}^{(L)}_k = \sum_{q \in \mathcal{W}_k}\sigma_q \D_q\g_q \label{c_final_eq}
\end{align}
where $\sigma_q = \frac{\sqrt{ 2\pi \delta_q \frac{\delta_q}{\Delta_k}}}{L \sum_{p=1}^{2^B}\delta_p} = \frac{\delta_q}{L\sqrt{2\pi\Delta_k}}$, noting that it holds that, 

% $$\mathbf{D D}^{H}=\left({L \sum_{p=1}^{2^B}\delta_p}\right) \mathbf{I}_{M_{t}}$$.
% % Dividing by $\|\Tilde{\c}^{(L)}_q\|$ and taking the limit as L goes to infinity we will find the optimal $\c_q$. i.e. 


Using \eqref{c_final_eq}, equation \eqref{g_final_eq} can now be rewritten as, 

\begin{align}
 &\mathcal{G}_k = \underset{\mathcal{G}}{\arg\min } \nonumber
 \\&\left\| abs(\D^H \D\sum_{q \in \mathcal{W}_k}\sigma_q(\mathbf{e}_{q} \otimes \mathbf{g}_q))-abs(\sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}(\mathbf{e}_{q} \otimes \mathbf{g}_q))\right\|^{2} \label{g_simple_final_eq}
\end{align} 

% where $\sigma' = \frac{1}{2\pi L}$. We will state the following theorem without formal proof.
\begin{proposition}
The maximizer of \eqref{g_simple_final_eq} is in the form $\g_q = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ for some $\eta$ where $\alpha = e^{j(\frac{\delta_q}{L})}$. \label{proposiiton_g}
\end{proposition}

An analytical closed form solution for $\c_q$ can be found as follows. We have, 
 \begin{align}
     {\c_k}^{(L)} & = \sum_{q \in \mathcal{W}_k} \sigma_q \left(\sum_{l=1}^{L}g_{q, l}\mathbf{d}_{M_t}(\psi_{q, l})\right)  \nonumber\\
     & = \sum_{q \in \mathcal{W}_k} \left(\sum_{l=1}^L \sigma_qg_q^{(l)}\left[{\begin{array}{ccc}
     1 &\cdots & e^{j(M_t-1)\psi_{q, l}}\\
     \end{array}}\right]^T \right)  \nonumber\\
     & = \sum_{q \in \mathcal{W}_k} \sigma_q \left[{\begin{array}{ccc}
     \sum_{l=1}^L g_{q, l}& \cdots & \sum_{l=1}^L g_{q, l}e^{j(M_t-1)\psi_{q, l}}\\
     \end{array}}\right]^T 
\end{align}

 
Let us write, 

\begin{equation}
    \c_k^{(L)} = \sum_{q \in \mathcal{W}_k} \c_q^{(L)}
\end{equation}

where, 

\begin{equation}
{\c_q}^{(L)}  = \sigma_q \sum_{l=1}^{L}g_{q, l}\mathbf{d}_{M_t}(\psi_{q, l})
\end{equation}


Choosing $\g_q$ as in proposition \ref{proposiiton_g},  the $m$-th element of the vector ${\c}_q = \lim_{L\rightarrow \infty}{\c_q}^{(L)} $, i.e. $c_{q,m}$, is given by 

\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}\lim_{L\rightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_{q, l} e^{j(m\psi_{q, l+1})}
\end{equation}

% With a choice of $\g_q = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ where we set 
% % $\alpha = e^j(\frac{2\pi}{L2^B})$
% $\alpha = e^{j(\frac{\delta_q}{L})}$ and suitable $\eta$ (to be determined later), we can write


% \begin{equation}
%     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{2 \pi(\ell+0.5)}{L2^B})}
% \end{equation}

\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}\lim_{L\rightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_{q, l} e^{jm(\psi_{q-1}+\frac{\delta_q(\ell+0.5)}{L})}
\end{equation}

% After some basic manipulations we get, 
\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}\lim_{L\rightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l} e^{jm(\psi_{q-1}+\frac{0.5\delta_q}{L})} 
\end{equation}


\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{jm(\psi_{q-1})}\lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l}   
\end{equation}

\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{jm(\psi_{q-1})} \int_{0}^{1} \alpha^{(\eta + m)Lx}dx
\end{equation}


\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\frac{2\pi(\eta + m)L}{L2^B}x}dx
\end{equation}


\begin{align}
 c_{q,m} &= \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{jm\psi_{q-1}} \int_{0}^{1} e^{j\xi x}dx \nonumber \\
 &= \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi}) \label{final_g}
\end{align}

where $\xi = \delta_q (\eta +m )$.


% \begin{equation}
%     c_{q,m} = e^{jm(\psi_{q-1})} \frac{e^{j\xi}-1}{j\xi}
% \end{equation}

% \begin{equation}
%     c_{q,m} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} \frac{e^{j\xi/2}-e^{-j\xi/2}}{j\xi/2}
% \end{equation}

% \begin{equation}
%     c_{q,m} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi}) \label{final_g}
% \end{equation}






% Note that the solution to part \textit{(a)} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity.
%  \begin{align}
% & \Tilde{\c}^{(L)}_q = (\D \D^H)^{-1} \D \sigma \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
% & \Tilde{\c}^{(L)}_q =  \sigma' \D \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) = \sigma' \D_q\g_q
% \end{align}
% Dividing by $\|\Tilde{\c}^{(L)}_q\|$ and taking the limit as L goes to infinity we will find the optimal $\c_q$. i.e. 

% \begin{equation}
%     \c_q = \lim_{L\longrightarrow \infty} \frac{\Tilde{\c}^{(L)}_q}{L\|\Tilde{\c}^{(L)}_q\|}
% \end{equation}

% We aim to find $\g_q$ such that

% \begin{align}
% & \left\| abs(\D^H \gamma' \D_q \mathbf{g}_q)- abs(\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)) \right\|_{2}^{2}
% \end{align}

% is minimized.

% % Is it possible to show that $\g_q$ is independent of $q$ (assume regular scenario)? If true, i.e., $\g_q = \g$ we have

% We will provide a suboptimal structure for the choice of $\g$. Let us assume $\g_q = \g, $  for all $ q \in \{1, \cdots, Q\}$. Then we can write
% \begin{align}
%      &\Tilde{\c_q}^{(L)} = D_q\mathbf{g} = \sum_{l=1}^{L}g_l\mathbf{d}_{M_t}(\psi_{q, l})  \nonumber\\
%      & = \sum_{l=1}^L g_l\left[{\begin{array}{cccc}
%      1& e^{j\psi_{q, l}} &\cdots & e^{j(M_t-1)\psi_{q, l}}\\
%      \end{array}}\right]^T  = \nonumber\\
%      & \left[{\begin{array}{cccc}
%      \sum_{l=1}^L g_l& \sum_{l=1}^L g_le^{j\psi_{q, l}} &\cdots & \sum_{l=1}^L g_le^{j(M_t-1)\psi_{q, l}}\\
%      \end{array}}\right]^T
%  \end{align}
 
 

%  We have for the $m$-th element of the vector $\Tilde{\c}_q$, i.e. $\Tilde{c}^{(m)}_q$  for $ 0 \leq m \leq M_t-1$

% \begin{equation}
%     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{j(m\psi_{q, l+1})}
% \end{equation}

% With a choice of $\g = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ where we set 
% % $\alpha = e^j(\frac{2\pi}{LQ})$
% $\alpha = e^j(\frac{\psi_{q}-\psi_{q-1}}{L})$ and suitable $\eta$ (to be determined later), we can write


% % \begin{equation}
% %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{2 \pi(\ell+0.5)}{LQ})}
% % \end{equation}

% \begin{equation}
%     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{(\psi_{q}-\psi_{q-1})(\ell+0.5)}{L})}
% \end{equation}

% \begin{equation}
%     c_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l} e^{jm(\psi_{q-1}+\frac{0.5(\psi_{q}-\psi_{q-1})}{L})} 
% \end{equation}


% \begin{equation}
%     c_q^{(m)} = e^{jm(\psi_{q-1})}\lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l}   
% \end{equation}

% \begin{equation}
%     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} \alpha^{(\eta + m)Lx}dx
% \end{equation}


% % \begin{equation}
% %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\frac{2\pi(\eta + m)L}{LQ}x}dx
% % \end{equation}


% \begin{equation}
%     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\xi x}dx
% \end{equation}

% where $\xi = (\psi_{q}-\psi_{q-1}) (\eta +m )$.


% \begin{equation}
%     c_q^{(m)} = e^{jm(\psi_{q-1})} \frac{e^{j\xi}-1}{j\xi}
% \end{equation}

% \begin{equation}
%     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} \frac{e^{j\xi/2}-e^{-j\xi/2}}{j\xi/2}
% \end{equation}

% \begin{equation}
%     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi})
% \end{equation}

% where, $sinc(t) = \frac{sin(\pi t)}{\pi t}$.
















% We first optimize for $\alpha$ by setting the derivative of \eqref{obj_func} to zero, to get: 

% $$\hat{\alpha}=\frac{\sum_{q \in \mathcal{W}_k}\sqrt{\frac{Q}{M_{t}}}(\mathbf{F} \mathbf{v})^{H} \mathbf{D}_{q} \mathbf{g}_q}{\left\|\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right\|_{2}^{2}}$$

% Replacing the value of $\alpha$ as above we get to the following optimization problem. 

% \begin{align}
% \left(\mathbf{F}_{\mid \mathbf{g}}, \mathbf{v}_{\mid \mathbf{g}}\right) &=\underset{\mathbf{F}, \mathbf{v}}{\arg \max } \frac{\left|\sum_{q \in \mathcal{W}_k}\sqrt{\frac{2^{\mathbf{B}}}{M_{t}}}\left(\mathbf{D}_{q} \mathbf{g}_q\right)^{H} \mathbf{F} \mathbf{v}\right|^{2}}{\left\|\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right\|_{2}^{2}} \nonumber \\
% &=\underset{\mathbf{F}, \mathbf{v}}{\arg \max }\left|\sum_{q \in \mathcal{W}_k}\left(\mathbf{D}_{q} \mathbf{g}\right)^{H} \mathbf{F} \mathbf{v}\right|^{2}
% \end{align}


% \section{Codebook Design Problem Formulation}
% \label{sec: formulation}

% % Let $\mathbf{c} \doteq \mathbf{F} \mathbf{v} \in \mathbb{C}^{M_{t}}$ be the unit-norm transmit beam-forming codeword, where analog beamsteering matrix $\mathbf{F}=\left[\mathbf{f}_{1}, \cdots, \mathbf{f}_{N_{R F}}\right] \in \mathbb{C}^{M_{t} \times N_{R F}}$ contains $N_{RF}$ equal-gain analog beamsteering vectors $\mathbf{f}_{n}$ and the baseband beamforming vector $\mathbf{v} \in \mathbb{C}^{N_{R F}}$ is such that $\|\c\|_{2}=1$ holds. The equal-gain constraint holds if $\mathbf{f}_{n} \in \mathcal{B}_{M_{t}}$ for 

% % \begin{equation}
% %     \mathcal{B}_{M_{t}}=\left\{\mathbf{w} \in \mathbb{C}^{M_{t}}:\left(\mathbf{w} \mathbf{w}^{H}\right)_{\ell, \ell}=1 / M_{t}, 1 \leq \ell \leq M_{t}\right\}
% %     \label{f_constant_gain}
% % \end{equation}

% % Let $\mathcal{C}=\left\{\mathbf{c}_{1}, \cdots, \mathbf{c}_{Q}\right\}$ be the codebook with codewords taking value as $\mathbf{c}_{q}=\mathbf{F}_{q} \mathbf{v}_{q}$. Consider a half-wavelength uniform linear array (ULA) of antennas as in the previous subsection, i.e. $d = \frac{\lambda}{2}$, with an array response vector as in \eqref{array_factor}.

% % % %$$\mathbf{d}_{M_{t}}(\psi)=\frac{1}{\sqrt{M_{t}}}\left[1 e^{j \psi} \cdots e^{j\left(M_{t}-1\right) \psi}\right]^{T} \in \mathbb{C}^{M_{t}}$$
% % % $$\mathbf{d}_{M_{t}}(\psi)=\left[1, e^{j \psi}, \cdots, e^{j\left(M_{t}-1\right) \psi}\right]^{T} \in \mathbb{C}^{M_{t}}$$

%  For convenience, in this section, we will drop the index \emph{ula} from the expression of the array factor $\d_{ula, M_t}(\psi)$ and gain $G^{ula}(\psi, \mathbf{c})$.  Before presenting the formulation of the codebook design problem, we introduce some new notations. We divide the angular range of $\theta \in [-\pi, 0]$  into equal-length beams $\omega_{q} \text { for } q \in\left\{1, \cdots, Q\right\}$. i.e. 
% $$
% \begin{aligned}
% \omega_{q} &=\left[\theta_{q-1}, \theta_{q}\right) ,& \theta_{q}= -\pi+ \frac{ \pi}{Q} q
% \end{aligned}
% $$

% % Further we introduce the change of variable $\psi = \frac{2 \pi d}{\lambda} \cos(\theta)$ where $\psi \in [-\pi, \pi]$. For $d = \frac{\lambda}{2}$,

% Corresponding to $\omega_q$ intervals, there exists $\nu_q$ ranges with respect to $\psi$ such that, 

% $$
% \begin{aligned}
% \nu_{q} &=\left[\psi_{q-1}, \psi_{q}\right), & \psi_q = -\pi\cos(\frac{\pi}{Q}q)
% \end{aligned}
% $$


% Under the reference gain as in \eqref{reference gain} and using Parseval's theorem \cite{parseval}, we will have:
% % and assuming $|\c| = 1$
% \begin{equation}
% \int_{-\pi}^{\pi} G(\psi, \mathbf{c}) d \psi=2 \pi\left\| \mathbf{c}\right\|^{2}=2 \pi\label{parseval}
% \end{equation}

% Let  $G_{\text {ideal }, q}(\psi)$ denote the desired ideal gain which is supposed to be constant on $\nu_q$ and zero otherwise. It must hold that, 
% % \begin{equation}
% % \int_{-\pi}^{\pi} G(\psi, \mathbf{c}) d \psi=2 \pi\left\|\frac{1}{\sqrt{M_{t}}} \mathbf{c}\right\|_{2}^{2}=\frac{2 \pi}{M_{t}}    \label{parseval}
% % \end{equation}





% \begin{align}
% &\int_{-\pi}^{\pi} G_{\text {ideal }, q}(\psi) d \psi =\int_{\nu_{q}} t d \psi+\int_{[-\pi, \pi] \backslash \nu_{q}} 0 d \psi \nonumber\\
% &=(\psi_q - \psi_{q-1}) t={2 \pi} \label{plain}
% \end{align}

% which in turn will give: 

% \begin{equation}
%     G_{\text {ideal }, q}(\psi)=\frac{2\pi}{(\psi_q - \psi_{q-1})} \mathds{1}_{\nu_{q}}(\psi), \quad \psi \in[-\pi, \pi] \label{ideal_gain}
% \end{equation}

% We aim to design the codebooks so as to mimic the ideal gain computed in equation \eqref{ideal_gain}. Therefore, the plain codebook design problem is formulated as a minimization of a MSE as follows: 


% % \begin{align}
% % &\left(\mathbf{F}_{\text {opt }, q}, \mathbf{v}_{\mathrm{opt}, q}\right) \nonumber \\&=\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \int_{-\pi}^{\pi}\left|G_{\text {ideal }, q}(\psi)-G(\psi, \mathbf{F} \mathbf{v})\right|^{2} d \psi
% % \end{align}

% \begin{align}
% &\c_q^{opt}=\underset{\c, \|\c\|=1}{\arg \min } \int_{-\pi}^{\pi}\left|G_{\text {ideal }, q}(\psi)-G(\psi, \c)\right| d \psi
% \label{composite_MSE}
% \end{align}

% By uniformly sampling on the range of $\psi$ we can rewrite the optimization problem as follows, 
% \begin{align}
%     &\underset{\c, \|\c\|=1}{\arg \min }\left[\lim _{L \rightarrow \infty} \sum_{p=1}^{Q} \delta_p \sum_{\ell=1}^{L} \frac{\left|G_{\text {ideal }, q}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \c \right)\right|}{L}\right]\label{equivalent_MSE}
% \end{align}

%  where for $q = 1 \ldots Q$, 
%  $$\delta_q = \psi_{q}-\psi_{q-1}, \quad \psi_{q, \ell}=\psi_{q-1}+\frac{\delta_q(\ell-0.5)}{L} $$

 
%  We can write equation \eqref{equivalent_MSE}, as 
%  \begin{align}
%  &\c_q^{opt} = \underset{\c,  \|\c\|=1}{\arg \min } \lim_{L\rightarrow \infty}\frac{1}{L}\left\|\mathbf{G}_{\text {ideal }, q}-\mathbf{G}(\c)\right\| \label{init_opt}
%  \end{align}
 
%  where,  $$\mathbf{G}(\c)=\left[{\delta_1} G\left(\psi_{1,1}, \c\right) \ldots {\delta_{Q}}G\left(\psi_{Q, L}, \c\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% and, 
% $$ \mathbf{G}_{\text {ideal }, q}=\left[{\delta_1} G_{\text {ideal }, q}\left(\psi_{1,1}\right) \ldots {\delta_{Q}}G_{\text {ideal }, q}\left(\psi_{Q, L}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% Note that it holds that 

% \begin{equation}
%     \mathbf{G}_{\text {ideal }, q}={2\pi}\left(\mathbf{e}_{q} \otimes \mathbf{1}_{L, 1}\right) \label{ideal}
% \end{equation}

% with $\mathbf{e}_{q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $q$-th axis among $Q$ ones. Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any equal gain $\mathbf{g} \in \mathbb{C}^L$. Therefore, for a suitable choice of $\g$ we can write: 

% % $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$


% \begin{align}
% \mathbf{G}_{\text {ideal }, q} &={2\pi}\left(\mathbf{e}_{q} \otimes\left(\mathbf{g} \odot \mathbf{g}^{*}\right)\right) \nonumber\\
% &=\left(\sqrt{2\pi}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right)\right) \odot\left(\sqrt{{2\pi}}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right)\right)^{*} \label{g_id_q_equivalent}
% \end{align}


% Similarly, it is straightforward to observe,


% \begin{align}
% \mathbf{G}(\c) &=\left(\mathbf{D}^{H} \c\right) \odot\left(\mathbf{D}^{H} \c\right)^{*} \label{dc}
% \end{align}
% where $\mathbf{D} =\left[\sqrt{\delta_1}\mathbf{D}_{1} \cdots \sqrt{\delta_{Q}}\mathbf{D}_{Q} \right] \in \mathbb{C}^{M_{t} \times L Q}$, and 
% $\mathbf{D}_{q}=\left[\mathbf{d}_{M_{t}}\left(\psi_{q, 1}\right) \cdots \mathbf{d}_{M_{t}}\left(\psi_{q, L}\right)\right] \in \mathbb{C}^{M_{t} \times L}.$
 

% % Comparing the expressions in equations \eqref{g_id_q_equivalent} and \eqref{dc},  we formulate the following two-step optimization for the codebook design problem for hybrid beamforming, presented below as \textit{Problem \ref{main_problem}}. Given a suitable $\g_q$, in the first step, we search for a unit-norm codeword $\c_q$ for fully-digital beamforming, and in the second step we find a suitable pair $(\F_q, \v_q)$ to complete the hybrid beamforming codebook design.  

 

% % \begin{problem}

% % a) For all $q \in \{1, \cdots, Q\}$, given equal-gain $\g_q \in \mathbb{C}^L$, find vector $\c_q \in \mathbb{C}^{M_t}$ such that
% % \begin{align}
% % &\c_q=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\longrightarrow \infty} \left\|\sqrt{2\pi}\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)- \mathbf{D}^{H} \c\right\|^{2} \label{obj_func}
% % \end{align}

% % \vspace{2mm}
% % \noindent
% % b) Find $\F_q \in \mathbb{C}^{M_t \times N_{RF}}$ , and $\v_q \in \mathbb{C}^{N_{RF}}$ that solve $\mathbf{F}_{q}\mathbf{v}_{q} = \c_q$ subject to the equal-gain condition on the columns of $\F_q$. 

% % % \begin{align}
% % %     \mathbf{F}_{\mid \g_q}\mathbf{v}_{\mid \g_q} = \c_q
% % % \end{align}
% % \label{main_problem}
% % \end{problem}

% % The solution to the last problem provides the optimal codebook designed for hybrid beamforming under a ULA structure, given the choice of $\g_q$. Note that we were initially trying to solve the optimization problem in equation \eqref{init_opt}. In light of modifications \eqref{g_id_q_equivalent}, and \eqref{dc}, the quantity to be minimized in the limit of equation \eqref{init_opt} can be written as follows,

% % \begin{align}
% %     & \left\|\mathbf{G}_{\text {ideal }, q}-\mathbf{G}(\c)\right\| = \left\| abs(\D^H \c_q)- \sqrt{2\pi} abs(\mathbf{e}_{q} \otimes \mathbf{g})\right\| \label{g_init}
% % \end{align}
% % where $abs(.)$ denotes the element-wise absolute value of a vector.

% % Equation \eqref{g_init} reveals the central role of the vector $\g_q$ in minimizing the MSE in equation \eqref{init_opt}. In fact, the choice of $\g_q$ has to be optimized in a way that norm in \eqref{g_init} is minimized; i.e. the result gain designed by codebook $\c_q$ gets as close as possible to the ideal gain. To optimize the choice of $\g_q$, we formulate the following optimization problem, presented as \textit{Problem \ref{g_problem}}.

% % \begin{problem}
% % For all $q = 1, \ldots, Q$, find equal-gain $\g_q \in \mathbb{C}^L$ such that

% % \begin{equation}
% %  \g_q = \underset{\g}{\arg\min }\left\| abs(\D^H \c_q)- \sqrt{2\pi} abs(\mathbf{e}_{q} \otimes \mathbf{g})\right\|^{2} \label{g_final_eq}
% % \end{equation} 

% % \label{g_problem}
% % \end{problem}

% % In the next session we propose our approach to solve problems \ref{main_problem} and \ref{g_problem}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comparing the expressions \eqref{init_opt}, \eqref{g_id_q_equivalent}, and \eqref{dc}, one can show that the optimal choice of $\c_q$ in \eqref{init_opt} is the solution to the following optimization problem for a proper choice of $\g_q$. 
% \begin{problem}
% Given an equal-gain vector $\g_q \in \mathbb{C}^L$, $q \in \{1, \cdots, Q\}$, find vector $\c_q \in \mathbb{C}^{M_t}$ such that
% \begin{align}
% &\c_q=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\longrightarrow \infty} \left\|\sqrt{2\pi}\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)- \mathbf{D}^{H} \c\right\|^{2} \label{obj_func}
% \end{align}
% \label{main_problem}
% \end{problem}
% However, we now need to find the optimal choice of $\g_q$ that minimizes the objective in \eqref{init_opt}. Using \eqref{g_id_q_equivalent}, and \eqref{dc}, we have the following optimization problem.
% \begin{problem}
% Find equal-gain $\g_q \in \mathbb{C}^L$, $q = 1, \ldots, Q$, such that
% \begin{equation}
%  \g_q = \underset{\g}{\arg\min }\left\| abs(\D^H \c_q)- \sqrt{2\pi} abs(\mathbf{e}_{q} \otimes \mathbf{g})\right\|^{2} \label{g_final_eq}
% \end{equation} 
% where $abs(.)$ denotes the element-wise absolute value of a vector.
% \label{g_problem}
% \end{problem}

% Hence, the codebook design for a system with full-digital beamforming capability is found by solving Problem~\ref{main_problem} for proper choice of $\g_q$ obtained as a solution to Problem ~\ref{g_problem}. The codebook for Hybrid beamforming, is then found as
% \begin{align}
%     \underset{\mathbf{F}_{q},\mathbf{v}_{q}}{\arg\min } \|\mathbf{F}_{q}\mathbf{v}_{q} - \c_q\|^2
% \end{align}
% where the columns of $\F_q \in \mathbb{C}^{M_t \times N_{RF}}$ are equal-gain vectors and $\v_q \in \mathbb{C}^{N_{RF}}$. The solution may be obtained using simple, yet effective suboptimal algorithm such as orthogonal matching pursuit (OMP) \cite{love15}\cite{noh17}\cite{Hussain17}. In the next section we continue with the solution of Problem~\ref{main_problem}, and~\ref{g_problem}.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % Note that the solution to part \textit{(a)} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity.
% %  \begin{align}
% % & \Tilde{\c}^{(L)}_q = (\D \D^H)^{-1} \D \sigma \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
% % & \Tilde{\c}^{(L)}_q =  \sigma' \D \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) = \sigma' \D_q\g_q
% % \end{align}
% % Dividing by $\|\Tilde{\c}^{(L)}_q\|$ and taking the limit as L goes to infinity we will find the optimal $\c_q$. i.e. 

% % \begin{equation}
% %     \c_q = \lim_{L\longrightarrow \infty} \frac{\Tilde{\c}^{(L)}_q}{L\|\Tilde{\c}^{(L)}_q\|}
% % \end{equation}

% % We aim to find $\g_q$ such that

% % \begin{align}
% % & \left\| abs(\D^H \gamma' \D_q \mathbf{g}_q)- abs(\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)) \right\|_{2}^{2}
% % \end{align}

% % is minimized.

% % % Is it possible to show that $\g_q$ is independent of $q$ (assume regular scenario)? If true, i.e., $\g_q = \g$ we have

% % We will provide a suboptimal structure for the choice of $\g$. Let us assume $\g_q = \g, $  for all $ q \in \{1, \cdots, Q\}$. Then we can write
% % \begin{align}
% %      &\Tilde{\c_q}^{(L)} = D_q\mathbf{g} = \sum_{l=1}^{L}g_l\mathbf{d}_{M_t}(\psi_{q, l})  \nonumber\\
% %      & = \sum_{l=1}^L g_l\left[{\begin{array}{cccc}
% %      1& e^{j\psi_{q, l}} &\cdots & e^{j(M_t-1)\psi_{q, l}}\\
% %      \end{array}}\right]^T  = \nonumber\\
% %      & \left[{\begin{array}{cccc}
% %      \sum_{l=1}^L g_l& \sum_{l=1}^L g_le^{j\psi_{q, l}} &\cdots & \sum_{l=1}^L g_le^{j(M_t-1)\psi_{q, l}}\\
% %      \end{array}}\right]^T
% %  \end{align}
 
 

% %  We have for the $m$-th element of the vector $\Tilde{\c}_q$, i.e. $\Tilde{c}^{(m)}_q$  for $ 0 \leq m \leq M_t-1$

% % \begin{equation}
% %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{j(m\psi_{q, l+1})}
% % \end{equation}

% % With a choice of $\g = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ where we set 
% % % $\alpha = e^j(\frac{2\pi}{LQ})$
% % $\alpha = e^{j(\frac{\psi_{q}-\psi_{q-1}}{L})}$ and suitable $\eta$ (to be determined later), we can write


% % % \begin{equation}
% % %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{2 \pi(\ell+0.5)}{LQ})}
% % % \end{equation}

% % \begin{equation}
% %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{(\psi_{q}-\psi_{q-1})(\ell+0.5)}{L})}
% % \end{equation}

% % \begin{equation}
% %     c_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l} e^{jm(\psi_{q-1}+\frac{0.5(\psi_{q}-\psi_{q-1})}{L})} 
% % \end{equation}


% % \begin{equation}
% %     c_q^{(m)} = e^{jm(\psi_{q-1})}\lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l}   
% % \end{equation}

% % \begin{equation}
% %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} \alpha^{(\eta + m)Lx}dx
% % \end{equation}


% % % \begin{equation}
% % %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\frac{2\pi(\eta + m)L}{LQ}x}dx
% % % \end{equation}


% % \begin{equation}
% %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\xi x}dx
% % \end{equation}

% % where $\xi = (\psi_{q}-\psi_{q-1}) (\eta +m )$.


% % \begin{equation}
% %     c_q^{(m)} = e^{jm(\psi_{q-1})} \frac{e^{j\xi}-1}{j\xi}
% % \end{equation}

% % \begin{equation}
% %     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} \frac{e^{j\xi/2}-e^{-j\xi/2}}{j\xi/2}
% % \end{equation}

% % \begin{equation}
% %     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi})
% % \end{equation}

% % where, $sinc(t) = \frac{sin(\pi t)}{\pi t}$.

% % \subsection{Twin-ULA Setting}

% % We start from problem \eqref{main_problem}, and particularly, equation \eqref{obj_func}. Let $\{\s_m\}_{m =0}^{M_t -1}$ denote the columns of $D^H$. We can write: 

% % \begin{align}
% % &\s_m c_q^{(m)} + \s_{m+M_t/2} c_q^{(m+M_t/2)} \nonumber\\
% % &= \s_m (c_q^{(m)} + e^{-j \frac{2\pi d_y}{\lambda} \sin(\theta)} c_q^{(m+M_t/2)}) \nonumber\\
% % & \approx \s_m \Tilde{c}_q^{(m)}, \quad  m = 0 \ldots \frac{M_t}{2}-1\end{align}

% % where we define 
% % \begin{equation}
% %     \Tilde{c}_q^{(m)} = c_q^{(m)} + e^{-j \frac{2\pi d_y}{\lambda} \sin(\theta^{(m)}_q)} c_q^{(m+M_t/2)} \label{c_defn}
% % \end{equation}

% % with $\theta_{q-1}\leq\theta^{(m)}_q \leq \theta_{q}$ being a constant value.  

% % Therefore, the solution to part $(a)$ of problem \eqref{main_problem}, under the twin-ULA setup can be expressed as:

% %  \begin{align}
% % & \Tilde{\c}_q = (\Tilde{\D} \Tilde{\D}^H)^{-1} \Tilde{\D} \sigma \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
% % & \Tilde{\c}_q =  \sigma' \Tilde{\D} \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) = \sigma' \Tilde{\D}_q\g_q
% % \end{align}

% % where it holds that $\Tilde{\D} \Tilde{\D}^H = \I_{\frac{M_t}{2}}$, and


% % $$\Tilde{\D}_{q}=\left[\d_{\frac{M_{t}}{2}}\left(\psi_{q, 1}\right) \cdots \d_{\frac{M_{t}}{2}}\left(\psi_{q, L}\right)\right] \in \mathbb{C}^{\frac{M_{t}}{2} \times L}$$

% % In other words, one can approximately think of the codebook design problem over a twin ULA of $M_t$ antennas, as such a problem over a ULA of size $\frac{M_t}{2}$.

% % Following the approach in the previous subsection, we can infer, 

% % \begin{equation}
% %     \Tilde{c}_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi}), \quad m = 0 \ldots \frac{M_t}{2} -1
% %     \label{twin_c_result}
% % \end{equation}

% % Having $d_y = \frac{\lambda}{3}$, equating equations \eqref{c_defn}, and \eqref{twin_c_result}, by further assuming $c_q^{(m + \frac{M_t}{2})} = e^{j\beta_m} c_q^{(m)}$, after basic operations we get: 

% % \begin{equation}
% %     c_q^{(m)} = \frac{e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi})}{1+ e^{-j(\frac{2\pi}{3}\sin(\theta_q^{(m)}) + \beta_m)}}
% % \end{equation}

% % % \begin{equation}
% % %     c_q^{(m)} = \frac{e^{j(m\psi_{q-1} + \frac{\xi}{2} +\frac{\pi}{3}\sin(\theta_q^{(m)})+\frac{\beta_m}{2}) sinc(\frac{\xi}{2\pi})}}{2\cos(\frac{\pi}{3}\sin(\theta_q^{(m)}) + \frac{\beta_m}{2})}
% % % \end{equation}

% % Therefore, for each codeword entry $c_q^{(m)}$, it remains to pick $\beta_m$ and $\theta_q^{(m)}$. We relax this decision by setting $\beta_m = \beta$, and $\theta_q^{(m)} = \theta_q$, $ m = 1 \ldots M_t$. Next we explicitly right the expression for the reference gain as $G(\theta, \c_{twin}) = \left|\d_{twin, M_{t}}^{H}(\theta) \c_{twin}\right|^{2}$ where 

% % \begin{align}
% %     &\d_{twin, M_{t}}(\theta) = \left[\d_{\frac{M_{t}}{2}}^{T}(\theta), e^{j(\frac{2\pi}{3}\sin(\theta))}\d_{\frac{M_{t}}{2}}^{T}(\theta)\right]^T\\
% %     & \c_{twin} = \left[\c^T_{twin, \frac{M_t}{2}}, e^{j\beta}\c^T_{twin, \frac{M_t}{2}}\right]^T
% % \end{align}

% % We can  therefore write, 

% % \begin{align}
% %     G(\theta, \c_{twin}) &= \left|\d_{\frac{M_{t}}{2}}^{H}(\theta)\c_{twin, \frac{M_t}{2}} (1 + e^{j(\beta-\frac{2\pi}{3}\sin(\theta))})\right|^2\nonumber\\
% %     & = \left|\d_{\frac{M_{t}}{2}}^{H}(\theta)\c\right|^2 \left| \frac{1 + e^{j(\beta-\frac{2\pi}{3}\sin(\theta))}}{1 + e^{-j(\beta+\frac{2\pi}{3}\sin(\theta))}}\right|^2
% % \end{align}

% % Further define 
% % $$ L(\theta) = \left| \frac{1 + e^{j(\beta-\frac{2\pi}{3}\sin(\theta))}}{1 + e^{-j(\beta+\frac{2\pi}{3}\sin(\theta))}}\right|$$
% % The last equation consists of two parts, the first part being the gain corresponding to a ULA of size $\frac{M_t}{2}$ and the second part being  $L^2(\theta)$. For any $\omega_q = \left[\theta_{q-1}, \theta_{q}\right)$, there exist a $\omega'_q \doteq \left(- \theta_{q}, -\theta_{q-1}\right]$. The gain of a ULA is symmetric over $\omega_q$, and $\omega'_q$ by definition. However utilizing a twin ULA we wish to suppress the gain over $\omega'_q$ as much as we can and contribute to the gain over $\omega_q$ for each codeword $c_q, \quad q = 1\ldots Q$. To this end, we define the \emph{isolation factor} $\mu$ as follows,

% % \begin{align}
% %     \mu = \underset{\omega_q}{\int}{\frac{L(-\theta)}{L(\theta)}} d\theta
% % \end{align}
% %  to denote the level of isolation between each $\omega_q$ and its counterpart.
 
 















% % % \subsection{Composite Codebook Design Problem}

% % % Let us define a \textit{composite beam} $\omega_k$ as a union of multiple disjoint, possibly non-neighboring beams $\nu_{q} \text { for } q \in \mathcal{Q} = \left\{1, \cdots, Q\right\}$. Let $\mathcal{C'}=\left\{\mathbf{c}_{1}, \cdots, \mathbf{c}_{K}\right\}$ be the codebook corresponding to the composite problem.

% % % % $$\bigcup_{k = 1}^{2^{B'}}{\omega_k} = [-\pi, \pi], \quad \text{and} \quad \omega_k \cap \omega_l = \emptyset, \quad \forall k\neq l.$$

% % % Moreover, define for each composite beam $\omega_k$ the set $\mathcal{W}_k \subseteq \mathcal{Q}$ to be the set of indices of the single beams that form $\omega_k$. i.e. $\mathcal{W}_k = \{q \in \mathcal{Q}: v_q \subseteq \omega_k\}$. 
% % % We have then for the new ideal gain for each new codeword $\textbf{c}_k$, 

% % % \begin{align}
% % % &\int_{-\pi}^{\pi} G_{\text {ideal }, k}(\psi) d \psi =\int_{\omega_{k}} t' d \psi+\int_{[-\pi, \pi] \backslash \omega_{k}} 0 d \psi \nonumber\\
% % % &= \sum_{q \in {\mathcal{W}_k}}{\int_{\nu_{q}} t' d \psi} = |\mathcal{W}_k|\frac{2 \pi}{Q} t'=\frac{2 \pi}{M_{t}} \label{composite}
% % % \end{align}

% % % Therefore, $t' = \frac{Q}{|\mathcal{W}_k| M_t}$. It follows that, 

% % % \begin{equation}
% % %     G_{\text {ideal }, k}(\psi)=\frac{Q}{|\mathcal{W}_k| M_{t}} \mathds{1}_{\omega_{k}}(\psi), \quad \psi \in[-\pi, \pi] \label{composite_ideal_gain}
% % % \end{equation}

% % % The new MSE problem for the $k$-th codeword can therefore be written as follows.

% % % \begin{align}
% % % &\left(\mathbf{F}_{\text {opt }, k}, \mathbf{v}_{\mathrm{opt}, k}\right) \nonumber \\&=\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \int_{-\pi}^{\pi}\left|G_{\text {ideal }, k}(\psi)-G(\psi, \mathbf{F} \mathbf{v})\right|^{2} d \psi \nonumber \\&= \underset{\mathbf{F}, \mathbf{v}}{\arg \min }\left[\lim _{L \rightarrow \infty} \sum_{p=1}^{Q} \sum_{\ell=1}^{L} \frac{\left|G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \mathbf{F} \mathbf{v}\right)\right|^{2}}{L Q / 2 \pi}\right]\label{composite_MSE}
% % % \end{align}


% % % \begin{align}
% % % \left(\mathbf{F}_{k}, \mathbf{v}_{k}\right) &=\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \sum_{p=1}^{Q} \sum_{\ell=1}^{L}\left|G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \mathbf{F} \mathbf{v}\right)\right|^{2} \nonumber\\
% % % &=\underset{\mathbf{F}, \mathbf{v}}{\arg \min }\lim_{L\longrightarrow \infty} \frac{1}{L}\left\|\mathbf{G}_{\text {ideal }, k}-\mathbf{G}(\mathbf{F} \mathbf{v})\right\|_{2}^{2} \label{init_opt}
% % % \end{align}

% % % where,  $$\mathbf{G}(\mathbf{F} \mathbf{v})=\left[G\left(\psi_{1,1}, \mathbf{F} \mathbf{v}\right) \cdots G\left(\psi_{Q, L}, \mathbf{F} \mathbf{v}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% % % and, 
% % % $$ \mathbf{G}_{\text {ideal }, k}=\left[G_{\text {ideal }, k}\left(\psi_{1,1}\right) \cdots G_{\text {ideal }, k}\left(\psi_{Q, L}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% % % Note that we can write using the definition of $\mathcal{W}_k$ that, 

% % % $$G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)=\left\{\begin{array}{ll}
% % % \frac{Q}{|\mathcal{W}_k| M_{t}}, & p \in \mathcal{W}_k \\
% % % 0, & p \notin \mathcal{W}_k 
% % % \end{array},\right.$$

% % % Or in the matrix form, 

% % % \begin{align}
% % %     &\mathbf{G}_{\text {ideal }, k}=\frac{Q}{|\mathcal{W}_k| M_{t}}\left((\bigoplus_{q \in \mathcal{W}_k}{\mathbf{e}_{q}}) \otimes \mathbf{1}_{L, 1}\right)  \nonumber \\ 
% % %     & = \sum_{q \in \mathcal{W}_k}{\frac{Q}{|\mathcal{W}_k| M_{t}}\left(\mathbf{e}_{q} \otimes \mathbf{1}_{L, 1}\right)} \label{G_ideal_k}
% % % \end{align}

% % % with $\mathbf{e}_{q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $q$-th axis among $Q$ ones. Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any $\mathbf{g} \in \mathcal{G}_L$, where, 

% % % $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$



% % % Therefore, equation \eqref{G_ideal_k} can be rewritten as:
% % % \begin{align}
% % % &\mathbf{G}_{\text {ideal }, k} = \sum_{q \in \mathcal{W}_k}\frac{Q}{|\mathcal{W}_k| M_{t}}\left(\mathbf{e}_{q} \otimes\left(\mathbf{g}_q \odot \mathbf{g}_q^{*}\right)\right) \nonumber\\
% % % &=\sum_{q \in \mathcal{W}_k}\left(\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right) \odot\left(\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)^{*} \nonumber\\
% % % &=\left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)  \odot \left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)^{*} \label{final_gik}
% % % \end{align}

% % % where $\sigma = \sqrt{\frac{Q}{|\mathcal{W}_k|M_{t}}}$. 
% % % On the other hand note that $\mathbf{G}(\mathbf{F} \mathbf{v})$ can be written as,


% % % \begin{equation}
% % %     \mathbf{G}(\mathbf{F} \mathbf{v}) =\left(\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right) \odot\left(\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right)^{*}\label{dfv_decomp}
% % % \end{equation}

% % % where, 
% % % $$\mathbf{D} =\left[\mathbf{D}_{1} \cdots \mathbf{D}_{Q}\right] \in \mathbb{C}^{M_{t} \times L Q}$$

% % % and, $\mathbf{D}_{q}=\left[\mathbf{d}_{M_{t}}\left(\psi_{q, 1}\right) \cdots \mathbf{d}_{M_{t}}\left(\psi_{q, L}\right)\right] \in \mathbb{C}^{M_{t} \times L}$. 

% % % Comparing the expressions in equations \eqref{final_gik}, and, \eqref{dfv_decomp}, a perfect solution to the optimization problem in \eqref{init_opt}, could be a pair $\textbf{(F, v)}$, for which the following equality holds.  



% % % \begin{align}
% % %     \mathbf{D}^{H} \mathbf{F} \mathbf{v}=\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right) \label{potential_answer}
% % % \end{align}

% % % However, we have that $M_t > N_{RF}$ and therefore, the matrix $\textbf{D}^H \textbf{F}$ may not be full-rank, resulting in the RHS of equation \eqref{potential_answer} being in the null space of LHS. Therefore, given some $\g_q \in \mathcal{G}_L$ we formulate the following two-step optimization problem to search for $\textbf{(F, v)}$ that gets as close as possible to the desired value. 

% % % \begin{problem}

% % % a) For all $q \in \{1, \cdots, Q\}$, given $\g_q \in \mathcal{G}_L$, find the unit-norm vector $\c_q \in \mathbb{C}^{M_t}$ such that
% % % \begin{align}
% % % &\c^{|\g_q}_q=\underset{\c}{\arg \min } \lim_{L\longrightarrow \infty} \frac{1}{L}\left\|\left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)- \mathbf{D}^{H} \c\right\|_{2}^{2} \label{obj_func}
% % % \end{align}

% % % \noindent
% % % b) For every given $\c_q$, find $\F_q \in \mathbb{C}^{M_t \times N_{RF}}$ , and $\v_q \in \mathbb{C}^{N_RF}$ that satisfy $\mathbf{F}_{q}\mathbf{v}_{q} = \c_q$ the condition $\f_n \in \mathcal{B}_{M_t}$ as in equation \eqref{f_constant_gain}. 

% % % % \begin{align}
% % % %     \mathbf{F}_{\mid \g_q}\mathbf{v}_{\mid \g_q} = \c_q
% % % % \end{align}

% % % \end{problem}

% % % Note that the solution to part \textit{(a)} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity.
% % %  \begin{align}
% % % & \Tilde{\c}^{(L)}_q = (\D \D^H)^{-1} \D \sigma \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
% % % & \Tilde{\c}^{(L)}_q =  \sigma' \D \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) = \sigma' \D_q\g_q
% % % \end{align}
% % % Dividing by $\|\Tilde{\c}^{(L)}_q\|$ and taking the limit as L goes to infinity we will find the optimal $\c_q$. i.e. 

% % % \begin{equation}
% % %     \c_q = \lim_{L\longrightarrow \infty} \frac{\Tilde{\c}^{(L)}_q}{L\|\Tilde{\c}^{(L)}_q\|}
% % % \end{equation}

% % % We aim to find $\g_q$ such that

% % % \begin{align}
% % % & \left\| abs(\D^H \gamma' \D_q \mathbf{g}_q)- abs(\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)) \right\|_{2}^{2}
% % % \end{align}

% % % is minimized.

% % % % Is it possible to show that $\g_q$ is independent of $q$ (assume regular scenario)? If true, i.e., $\g_q = \g$ we have

% % % We will provide a suboptimal structure for the choice of $\g$. Let us assume $\g_q = \g, $  for all $ q \in \{1, \cdots, Q\}$. Then we can write
% % % \begin{align}
% % %      &\Tilde{\c_q}^{(L)} = D_q\mathbf{g} = \sum_{l=1}^{L}g_l\mathbf{d}_{M_t}(\psi_{q, l})  \nonumber\\
% % %      & = \sum_{l=1}^L g_l\left[{\begin{array}{cccc}
% % %      1& e^{j\psi_{q, l}} &\cdots & e^{j(M_t-1)\psi_{q, l}}\\
% % %      \end{array}}\right]^T  = \nonumber\\
% % %      & \left[{\begin{array}{cccc}
% % %      \sum_{l=1}^L g_l& \sum_{l=1}^L g_le^{j\psi_{q, l}} &\cdots & \sum_{l=1}^L g_le^{j(M_t-1)\psi_{q, l}}\\
% % %      \end{array}}\right]^T
% % %  \end{align}
 
 

% % %  We have for the $m$-th element of the vector $\Tilde{\c}_q$, i.e. $\Tilde{c}^{(m)}_q$  for $ 0 \leq m \leq M_t-1$

% % % \begin{equation}
% % %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{j(m\psi_{q, l+1})}
% % % \end{equation}

% % % With a choice of $\g = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ where we set 
% % % % $\alpha = e^j(\frac{2\pi}{LQ})$
% % % $\alpha = e^j(\frac{\psi_{q}-\psi_{q-1}}{L})$ and suitable $\eta$ (to be determined later), we can write


% % % % \begin{equation}
% % % %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{2 \pi(\ell+0.5)}{LQ})}
% % % % \end{equation}

% % % \begin{equation}
% % %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{(\psi_{q}-\psi_{q-1})(\ell+0.5)}{L})}
% % % \end{equation}

% % % \begin{equation}
% % %     c_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l} e^{jm(\psi_{q-1}+\frac{0.5(\psi_{q}-\psi_{q-1})}{L})} 
% % % \end{equation}


% % % \begin{equation}
% % %     c_q^{(m)} = e^{jm(\psi_{q-1})}\lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l}   
% % % \end{equation}

% % % \begin{equation}
% % %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} \alpha^{(\eta + m)Lx}dx
% % % \end{equation}


% % % % \begin{equation}
% % % %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\frac{2\pi(\eta + m)L}{LQ}x}dx
% % % % \end{equation}


% % % \begin{equation}
% % %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\xi x}dx
% % % \end{equation}

% % % where $\xi = (\psi_{q}-\psi_{q-1}) (\eta +m )$.


% % % \begin{equation}
% % %     c_q^{(m)} = e^{jm(\psi_{q-1})} \frac{e^{j\xi}-1}{j\xi}
% % % \end{equation}

% % % \begin{equation}
% % %     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} \frac{e^{j\xi/2}-e^{-j\xi/2}}{j\xi/2}
% % % \end{equation}

% % % \begin{equation}
% % %     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi})
% % % \end{equation}

% % % where, $sinc(t) = \frac{sin(\pi t)}{\pi t}$.
















% % % % We first optimize for $\alpha$ by setting the derivative of \eqref{obj_func} to zero, to get: 

% % % % $$\hat{\alpha}=\frac{\sum_{q \in \mathcal{W}_k}\sqrt{\frac{Q}{M_{t}}}(\mathbf{F} \mathbf{v})^{H} \mathbf{D}_{q} \mathbf{g}_q}{\left\|\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right\|_{2}^{2}}$$

% % % % Replacing the value of $\alpha$ as above we get to the following optimization problem. 

% % % % \begin{align}
% % % % \left(\mathbf{F}_{\mid \mathbf{g}}, \mathbf{v}_{\mid \mathbf{g}}\right) &=\underset{\mathbf{F}, \mathbf{v}}{\arg \max } \frac{\left|\sum_{q \in \mathcal{W}_k}\sqrt{\frac{2^{\mathbf{B}}}{M_{t}}}\left(\mathbf{D}_{q} \mathbf{g}_q\right)^{H} \mathbf{F} \mathbf{v}\right|^{2}}{\left\|\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right\|_{2}^{2}} \nonumber \\
% % % % &=\underset{\mathbf{F}, \mathbf{v}}{\arg \max }\left|\sum_{q \in \mathcal{W}_k}\left(\mathbf{D}_{q} \mathbf{g}\right)^{H} \mathbf{F} \mathbf{v}\right|^{2}
% % % % \end{align}


% \subsection{UPA Codebook Design Prolem}

% Suppose an $M_h \times M_v$ UPA is placed at the $x-z$ plane, and let $M = M_h M_v$. Let the distance between the antennas that are placed parallel to $z$ axis, be $d_z$, and $d_x$ respectively. One can define,

% \begin{align}
% \mathbf{d}_{M_{a}}\left(\psi_{a}\right) = \left[1, e^{j \psi_{a}} \cdots e^{j\left(M_{a}-1\right) \psi_{a}}\right]^{T} \in \mathbb{C}^{M_{a}}
% \end{align}
% where, $\psi_{h}=\frac{2 \pi d_{x}}{\lambda} \sin \theta \cos \phi \text { and } \psi_{v}=\frac{2 \pi d_{z}}{\lambda} \sin \phi$, and $a$ takes value in the set $\{v, h\}$.  
% The array response vector is then defined as 

% \begin{align}
%     \mathbf{d}_{M}\left(\psi_{v}, \psi_{h}\right) =
%     \mathbf{d}_{M_{v}}\left(\psi_{v}\right) \otimes
%     \mathbf{d}_{M_{h}}\left(\psi_{h}\right)  \in \mathbb{C}^{M}
% \end{align}
% Let $\mathcal{B}_s$ be the angular range under cover. We have, 

% \begin{equation}
%     \mathcal{B}_{s} \doteq \left[-\phi^{\mathrm{B}}, \phi^{\mathrm{B}}\right)
%     \times \left[-\theta^{\mathrm{B}}, \theta^{\mathrm{B}}\right) \label{range_angle}
% \end{equation}

% Notation $\psi^{p,q}_{h}[1:L_h,1 :L_v], \psi^{p,q}_{v}[1:L_v]$

% Let us uniformly divide the angular range  into $Q=Q_{v} Q_{h}$ subregions. For each subregion we have, 

% $$ \mathcal{B}_{p, q} =  \omega_{\phi, p} \times \omega_{\theta, q}$$

% Let $\Delta_{\theta} =  2 \theta^{\mathrm{B}} / Q_{v}$, and $\Delta_\phi =  2 \phi^{\mathrm{B}} / Q_{h}$ be the length of each sub-interval along axis $\theta$, and $\phi$. We have $\omega_{\theta, q} = [\theta_{q-1}, \theta_q)$, and, $\omega_{\phi, p} = [\phi_{p-1},\phi_p)$ where  $\theta_q = -\theta^B + q\Delta_\theta$, and $\phi_p = -\phi^B + p\Delta_\phi$. 


% In the $(\psi_h, \psi_v)$ domain, we can rewrite equation \eqref{range_angle} as, 

% \begin{equation}
%     \mathcal{B}^\psi_{s} \doteq\left[-\psi_h^{\mathrm{B}}, \psi_h^{\mathrm{B}}\right) \times\left[-\psi_v^{\mathrm{B}}, \psi_v^{\mathrm{B}}\right)
% \end{equation}

% and each sub-region similarly can be rewritten in the $\psi$ domain as

% $$ \mathcal{B}^\psi_{ p, q} \doteq \nu_{v}^{p, q} \times \nu_{h}^ {p, q}$$

% % We can then write for each $v_{a, b}$, i.e the $b$-th sub-interval along axis $a$,

% % \begin{equation}
% %     \nu_{v, p} =-\psi_{a}^{\mathrm{B}}+(b-1)\Delta_{a}+\left[0, \Delta_{a}\right)
% % \end{equation}

% Define the reference gain at $(\psi_{h}, \psi_{v}) $ as, 

% \begin{equation}
%     G\left(\psi_{v}, \psi_{h}, \mathbf{c}\right) =\left|\left(\mathbf{d}_{M_{v}}\left(\psi_{v}\right)\otimes\mathbf{d}_{M_{h}}\left(\psi_{h}\right)  \right)^{H} \mathbf{c}\right|^{2}
% \end{equation}

% It is straightforward to show that, 

% \begin{equation}
%     \int_{-\pi}^{\pi} \int_{-\pi}^{\pi} G\left(\psi_{v}, \psi_{h}, \mathbf{c}\right) d \psi_{v} d \psi_{h}={(2 \pi)^{2}}
% \end{equation}

% Therefore, for every interval $\mathcal{B}_{ p, q}$ we can derive the ideal gain expression as, 

% \begin{equation}
%     G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)=G_{p,q} \mathds{1}_{\mathcal{B}^\psi_{p, q}}\left(\psi_{v}, \psi_{h}\right)
% \end{equation}

% where $G_{q,p} = \frac{(2\pi)^2}{\delta_{p,q}}$, where $\delta_{p,q}$ is the area of the interval $\mathcal{B}^\psi_{p,q}$. We define the codebook design problem under the UPA structure as follows. 
% % where $G_{q,p} = \frac{(2\pi)^2}{\delta^{p,q}_h\delta^p_v}$, $\delta^p_v = \psi^p_v - \psi^{p-1}_v $, and $\delta^{q, p}_h = \psi^{q,p}_h - \psi^{q-1, p}_h $. Also, let us define $\delta_{q,p} = \delta^{q, p}_h\delta^p_v$. 



% \begin{align}
% & \c^{opt}_{p, q} = \nonumber\\&\underset{\c, \|\c\|=1}{\arg \min } \iint_{\mathcal{B}_{s}}\left|G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)-G\left(\psi_{v}, \psi_{h}, \c\right)\right| d \psi_{v} d \psi_{h} \label{init_opt}
% \end{align}

% By partitioning the range of $(\psi_h, \psi_v)$ into the pre-defined intervals, we can rewrite the optimization problem as follows, 

% \begin{align}
% & \c^{opt}_{p, q} = \underset{\c, \|\c\|=1}{\arg \min }\nonumber\\& \sum_{r=1}^{Q_v}\sum_{s=1}^{Q_h}\iint_{\mathcal{B}^{\psi}_{r,s}}\left|G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)-G\left(\psi_{v}, \psi_{h}, \c\right)\right| d \psi_{v} d \psi_{h} \nonumber\\&
%  = \underset{L_h, L_v \rightarrow \infty}{\lim}\sum_{r=1}^{Q_v}\sum_{s=1}^{Q_h}\sum_{l_v =1}^{L_v}\sum_{l_h =1}^{L_h}\frac{\delta^r_v\delta^{r,s,l_v}_h}{L_hL_v}\nonumber\\&
% \left|G_{p, q}^{\text {ideal }}\left(\psi^{r,s}_{v}[l_v], \psi^{r,s}_{h}[l_v][l_h]\right)-G\left(\psi^{r,s}_{v}[l_v], \psi^{r,s}_{h}[l_v][l_h], \c\right)\right| \label{alternative_opt}
% \end{align}
% where, 

% \begin{align}
%     &\psi^{r,s}_v[l_v] = \psi^{r-1, s}_v + l_v\frac{\delta_v^r}{L_v}\nonumber\\
%     &\psi^{r,s}_h[l_v][l_h] = \psi^{r, s-1}_h[l_v] + l_h\frac{\delta_h^{r,s, l_v}}{L_h}
% \end{align}

% We can rewrite the optimization problem \eqref{alternative_opt} as, 

% \begin{align}
%     \c_{p,q}^{opt}=\arg \min _{\c, \|\c\|=1} \underset{L_h, L_v \rightarrow \infty}{\lim}\frac{1}{L_hL_v}\left\|\mathbf{G}^{\text {ideal }}_{p,q}-\mathbf{G}(\c)\right\|
% \end{align}


% where, 

% \begin{align}
%     &\mathbf{G}(\c) = \nonumber\\&\left[\delta^1_v\delta^{1,1,1}_hG\left(\psi_{v}^{1,1}[1], \psi_{h}^{1,1}[1][1], \c\right) \cdots \right. \nonumber\\ &\left. \delta^{Q_v}_v\delta^{Q_v,Q_h,L_v}_hG\left(\psi_{v}^{Q_{v}, Q_{h}}\left[L_{v}\right], \psi_{h}^{Q_{v}, Q_{h}}\left[L_{v}\right]\left[L_{h}\right], \c\right)\right]^{T} 
% \end{align}

% and, 

% \begin{align}
%     &\mathbf{G}^{\text {ideal }}_{ p, q} = \nonumber\\&\left[\delta^1_v\delta^{1,1,1}_hG^{\text {ideal }}_{ p, q}\left(\psi_{v}^{1,1}[1], \psi_{h}^{1,1}[1][1] \right) \cdots \right. \nonumber\\ &\left. \delta^{Q_v}_v\delta^{Q_v,Q_h,L_v}_hG^{\text {ideal }}_{ p, q}\left(\psi_{v}^{Q_{v}, Q_{h}}\left[L_{v}\right], \psi_{h}^{Q_{v}, Q_{h}}\left[L_{v}\right]\left[L_{h}\right]\right)\right]^{T} 
% \end{align}


% % \begin{align}
% %      &\mathbf{G}^{\text {ideal }}_{ q, p}= \nonumber\\&\left[{\delta_{1,1}} G^{\text {ideal }} _{q, p}\left(\psi^{1}_{h}[1], \psi^{1}_{v}[1], \c\right) \ldots {\delta_{Q_h, Q_v}}G^{\text {ideal }} _{q, p}\left(\psi^{Q_h}_{h}[L_h], \psi^{Q_v}_{v}[L_v], \c\right)\right]^{T} 
% % \end{align}


% Note that we can write, 

% \begin{align}
%     \mathbf{G}^{\text{ideal }}_{p,q} = \frac{{(2\pi)}^2}{\delta_{p,q}} \left(\e_{p,q} \otimes (\boldsymbol{\delta}_{p,q}\odot\mathbf{1}_{L, 1})\right)
% \end{align}

% where, $\boldsymbol\delta_{p,q} = $
% with $\mathbf{e}_{p,q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $(p,q)$-th axis among $Q$ ones. 








% Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any equal gain $\mathbf{g} \in \mathbb{C}^L$. Therefore, we can write: 

% % $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$


% \begin{align}
% \mathbf{G}^{\text {ideal }}_{p,q} &=\frac{{2\pi}^2}{\delta_{p,q}}\left(\mathbf{e}_{p,q} \otimes\left((\boldsymbol\delta^{(\frac{1}{2})}_{p,q}\odot\boldsymbol\delta^{(\frac{1}{2})}_{p,q})\odot(\mathbf{g} \odot \mathbf{g}^{*})\right)\right) \nonumber\\
% &=\left(\frac{{2\pi}}{\sqrt{\delta_{p,q}}}\left(\mathbf{e}_{p,q} \otimes (\boldsymbol\delta^{(\frac{1}{2})}_{p,q}\odot\mathbf{g})\right)\right) \nonumber\\&\odot\left(\frac{{(2\pi)}}{\sqrt{\delta_{p,q}}}\left(\mathbf{e}_{p,q} \otimes (\boldsymbol\delta^{(\frac{1}{2})}_{p,q}\odot\mathbf{g})\right)\right)^{*} \label{g_id_q_equivalent}
% \end{align}

% Also, note that we can write, 

% % \begin{align}
% %     \mathbf{G}(\c)=\left(\left(\mathbf{D}_{h}^{H} \otimes \mathbf{D}_{v}^{H}\right) \c\right) \odot\left(\left(\mathbf{D}_{h}^{H} \otimes \mathbf{D}_{v}^{H}\right) \c\right)^{*}
% % \end{align}
% \begin{align}
%     \mathbf{G}(\c)=\left(\D^H \c\right) \odot\left(\D^H \c\right)^{*}
% \end{align}

% where 

% \begin{align}
%     \D = \left[D^{1,1}_{vh}, \cdots, D^{Q_v,Q_h}_{vh}\right] \in \mathbb{C}^{M_vM_h\times L_vL_hQ_vQ_h}
% \end{align}

% % \begin{align}
% % % &\mathbf{D}_{v} =\left[\mathbf{D}_{v, 1}, \cdots, \mathbf{D}_{v, Q_{v}}\right] \in \mathbb{C}^{M_{v} \times L_{v} Q_{v}} \\
% % % &\mathbf{D}_{h} =\left[\mathbf{D}_{h, 1}, \cdots, \mathbf{D}_{h, Q_{h}}\right] \in \mathbb{C}^{M_{h} \times L_{h} Q_{h}} \\
% % % &\mathbf{D}_{v, p} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right)\right] \in \mathbb{C}^{M_{v} \times L_{v}}\\
% % % &\mathbf{D}_{h, q} =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1]\right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right]\right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% % &\mathbf{D}_{h, q}(\chi) =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1], \chi \right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right], \chi \right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% % &\mathbf{D}_{vh, p,q} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right) \otimes \mathbf{D}_{h, q}(\psi_{v}^{p}[1]), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right) \otimes \mathbf{D}_{h, q}(\psi_{v}^{p}\left[L_{v}\right]) \right] \in \mathbb{C}^{M_{v}M_{h} \times L_{v}L_{h}}
% % \end{align}

% \begin{align}
% % &\mathbf{D}_{v} =\left[\mathbf{D}_{v, 1}, \cdots, \mathbf{D}_{v, Q_{v}}\right] \in \mathbb{C}^{M_{v} \times L_{v} Q_{v}} \\
% % &\mathbf{D}_{h} =\left[\mathbf{D}_{h, 1}, \cdots, \mathbf{D}_{h, Q_{h}}\right] \in \mathbb{C}^{M_{h} \times L_{h} Q_{h}} \\
% % &\mathbf{D}_{v, p} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right)\right] \in \mathbb{C}^{M_{v} \times L_{v}}\\
% % &\mathbf{D}_{h, q} =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1]\right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right]\right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% \mathbf{D}^{p,q}_{h}(\ell) =&\sqrt{\delta_v^{p}\delta^{p,q,\ell}_h}\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{p,q}[\ell][1] \right), \cdots, \right.\nonumber\\&\left. \mathbf{d}_{M_{h}}\left(\psi_{h}^{p,q}\left[\ell] [L_{h} \right] \right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}, 
% \end{align}

% \begin{align}
%     \mathbf{D}_{vh}^{p,q} =&\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p,q}[1]\right) \otimes \mathbf{D}_{h}^{p,q}(1), \cdots, \right.\nonumber\\&\left. \mathbf{d}_{M_{v}}\left(\psi_{v}^{p,q}\left[L_{v}\right]\right) \otimes \mathbf{D}_{h}^{p,q}(L_{v}) \right] \in \mathbb{C}^{M_{v}M_{h} \times L_{v}L_{h}}
% \end{align}
% \begin{problem}
% Given an equal-gain vector $\g_{p,q} \in \mathbb{C}^L$, $(p,q) \in \{(1,1), \cdots, (Q_v, Q_h)\}$, find vector $\c_{p,q} \in \mathbb{C}^{M_t}$ such that
% \begin{align}
% &\c_{p,q}=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\rightarrow \infty} \left\|\frac{{2\pi}}{\sqrt{\delta_{p,q}}}\left(\mathbf{e}_{p,q} \otimes (\boldsymbol\delta^{(\frac{1}{2})}_{L,1}\odot\mathbf{g}_{p,q})\right)- \D^H \c\right\|^{2} \label{obj_func}
% \end{align}
% \label{main_problem_UPA}
% \end{problem}


% Note that the solution to problem \ref{main_problem_UPA} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity. For each $L$ we find that,
%  \begin{align}
%  {\c}^{(L)}_{p,q} &= {\frac{{2\pi}}{\sqrt{\delta_{p,q}}}}(\D \D^H)^{-1} \D  \left(\mathbf{e}_{p,q} \otimes (\boldsymbol\delta^{(\frac{1}{2})}_{L,1}\odot\mathbf{g}_{p,q})\right) \nonumber\\& =\sigma \D^{p,q}(\boldsymbol\delta^{(\frac{1}{2})}_{L,1}\odot\mathbf{g}_{p,q})
% \end{align}
% where $\sigma = \frac{2\pi \sqrt{\delta_{p,q}}}{L\sum_{(q,p)= (1,1)}^{(Q_h, Q_v)} \delta_{p,q}}$, noting that it holds that, 

% Noting that it holds that, 

% \begin{align}
%     (\D\D^H) = \left(L\sum_{(p,q)= (1,1)}^{(Q_h, Q_v)}\sum_{(l_v,l_h)= (1,1)}^{(L_h, L_v)} \delta_{v}^p\delta^{p,q,l_v}_{h}\right)\I_{M_t}
% \end{align}

% \begin{problem}
% Find equal-gain $\g_{p,q} \in \mathbb{C}^L$, $(q,p) = (1,1), \ldots, (Q_h, Q_v)$, such that
% \begin{equation}
%  \g_{q,p} = \underset{\g}{\arg\min }\left\| abs(\D^H \c_{q,p})- {2\pi} abs(\mathbf{e}_{q,p} \otimes \mathbf{g})\right\|^{2} \label{g_final_eq}
% \end{equation} 
% where $abs(.)$ denotes the element-wise absolute value of a vector.
% \label{g_problem}
% \end{problem}


% \begin{proposition}
% The minimizer of \eqref{g_simple_final_eq} is in the form $\g_q = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha_h^{\eta (L_h -1)}\alpha_v^{\eta (L_v -1)} \end{array}}\right]^T$ for some $\eta$ where $\alpha_h = e^{j(\frac{\delta^{q,p}_h}{L_h})}$ and $\alpha_v = e^{j(\frac{\delta^p_v}{L_v})}$. \label{proposiiton_g}
% \end{proposition}

%  \begin{align}
%      {\c_{p,q}}^{(L)} & = \sigma \sum_{(l_v, l_h)=(1,1)}^{(L_v, L_h)}g_{p,q, l}\mathbf{d}_{M_t}\left(\psi^{p,q}_{v}[l_v], \psi^{p,q}_{h}[l_v][l_h]\right)  \nonumber\\
%      & = \sigma \sum_{l=1}^L g_{q,p,l}\left[{\begin{array}{ccc}
%      1 &\cdots & e^{j\left( (M_v-1)\psi^{p,q}_{v}[l_v] + (M_h-1)\psi^{p,q}_{h}[l_v][l_h]\right)}\\
%      \end{array}}\right]^T   
%     %  \nonumber\\& = \left[{\begin{array}{ccc}
%     %  \sigma\sum_{l=1}^L g_{q, p, l}& \cdots & \sigma\sum_{l=1}^L g_{q,p, l}e^{j\left((M_h-1)\psi^q_{h}[l] + (M_v-1)\psi^p_{v}[l]\right)}\\
%     %  \end{array}}\right]^T
% \end{align}

% We can then write 

% \begin{align}
%     c_{p,q, m_v, m_h} &= \lim_{L_h, L_v\rightarrow \infty} \frac{1}{L_hL_v}\sum_{(l_h, l_v)=(1,1)}^{(L_h, L_v)} \nonumber \\&\delta^p_v\delta_h^{p,q,l_v}g_{p,q, l_v, l_h}e^{j\left(m_v\psi^{p,q}_{v}[l_v]+ m_h\psi^{p,q}_{h}[l_v][l_h] \right)}
% \end{align}


% \begin{align}
%     c_{p,q, m_v, m_h} &=  \nonumber\\&\lim_{L_h, L_v\rightarrow \infty} \frac{1}{L_hL_v}\sum_{(l_h, l_v)=(1,1)}^{(L_h, L_v)} \delta^p_v\delta_h^{p,q,l_v}g_{p,q, l_v, l_h}\nonumber \\&e^{j\left(m_v(\psi^{p-1,q}_{v}+l_v\frac{\delta^p_v}{L_v})+ m_h(\psi^{p,q-1}_{h}[l_v] + l_h\frac{\delta^{p,q,l_v}_h}{L_h}) \right)}
% \end{align}


% \begin{align}
%     c_{p,q, m_v, m_h} &=  \lim_{ L_v\rightarrow \infty} \frac{\delta^p_v}{L_v}\sum_{l_v=1}^{L_v} e^{j(m_v(\psi^{p-1,q}_{v}+l_v\frac{\delta^p_v}{L_v}) + x\eta\frac{l_v}{L_v})} S^{(l_v)}
% \end{align}

% where, 

% \begin{align}
%     S^{(l_v)} &= \lim_{ L_h\rightarrow \infty}\frac{\delta^{p,q,l_v}_h}{L_h}\sum_{l_h=1}^{L_h}e^{j(m_h(\psi^{p,q-1}_{h}[l_v] + l_h\frac{\delta^{p,q,l_v}_h}{L_h}) + y\gamma \frac{l_h}{L_h})} \nonumber\\& = \delta^{p,q,l_v}_h e^{jm_h\psi^{p,q-1}_{h}[l_v]}sinc(\frac{\xi}{2\pi})
% \end{align}

% with $\xi = {\delta^{p,q,l_v}_h}{m} + y\gamma$. Therefore, it. holds that, 

% \begin{align}
%     c_{p,q, m_v, m_h} &=  \lim_{ L_v\rightarrow \infty} \frac{\delta^p_v}{L_v}\sum_{l_v=1}^{L_v} e^{j(m_v(\psi^{p-1,q}_{v}+l_v\frac{\delta^p_v}{L_v}) + x\eta\frac{l_v}{L_v})} \delta^{p,q,l_v}_h e^{jm_h\psi^{p,q-1}_{h}[l_v]}sinc(\frac{\xi}{2\pi})
% \end{align}

==> related_work.tex <==
\section{Related Work}
\label{sec:relatedwork}
 
